A Review of Large Language Models and Autonomous Agents in Chemistry

Large language models (LLMs) have emerged as powerful tools in chemistry, significantly impacting molecule design, property prediction, and synthesis optimization. This review highlights LLM capabilities in these domains and their potential to accelerate scientific discovery through automation. We also review LLM-based autonomous agents: LLMs with a broader set of tools to interact with their surrounding environment. These agents perform diverse tasks such as paper scraping, interfacing with automated laboratories, and synthesis planning. As agents are an emerging topic, we extend the scope of our review of agents beyond chemistry and discuss across any scientific domains. This review covers the recent history, current capabilities, and design of LLMs and autonomous agents, addressing specific challenges, opportunities, and future directions in chemistry. Key challenges include data quality and integration, model interpretability, and the need for standard benchmarks, while future directions point towards more sophisticated multi-modal agents and enhanced collaboration between agents and experimental methods. Due to the quick pace of this field, a repository has been built to keep track of the latest studies: https://github.com/ur-whitelab/LLMs-in-science.

==> LLM_fig.tex <==
\begin{figure*}[h!]
    \begin{adjustbox}{width=\textwidth}
    \fontsize{4pt}{5pt}
        \begin{forest}
        for tree={
                forked edges,
                grow'=0,
                draw,
                rounded corners,
                node options={align=center},
                text width=2.7cm,
                s sep=6pt,
                calign=edge midpoint, 
            },
                [SciLLMs, fill=blue, root
                    [Text2Text, task
                        [Question-answering, application
                            [{BioMedLM\cite{Bolton2024-al}, BioMistral\cite{Labrak2024-xs}, BiMediX\cite{Pieri2024-jy}, EpilepsyLLM\cite{Zhao2024-hi}, CheXagent\cite{Chen2024-lg}, BioMedGPT-LM\cite{Luo2023-gw}, Darwin\cite{Xie2023-nh}, PMC-LLaMA\cite{Wu2023-tb}, Galactica\cite{Taylor2022-pu}, BioGPT\cite{Luo2022-sv}, nacho0\cite{Livne2023-bu}, etc.}, study]
                        ]
                    ]
                    [Text2Mol, task
                        [Conditional de-novo generation,  application
                            [{BioT5+\cite{Pei2024-ph}, Darwin\cite{Xie2023-nh}, Text+Chem T5\cite{Christofidellis2023-ea}, MolT5\cite{Edwards2022-yu}, etc.}, study]
                        ]
                    ]
                    [Text2Number, task
                        [Document classification, application
                            [{MatSciBERT\cite{Gupta2022-hy}, Galactica\cite{Taylor2022-pu}, PubMedBERT\cite{Gu2021-yn}, SciBERT\cite{Beltagy2019-ri}, BlueBERT\cite{Peng2019-yb}, etc}, study]
                        ]
                        [Property prediction, application
                            [{EpilepsyLLM\cite{Zhao2024-hi},             CatBERTa\cite{ock_catalyst_2023}, ScholarBERT\cite{Hong2022-mv}, ClinicalBERT\cite{Huang2019-gw}, etc}, study]
                        ]
                        [Named entity recognition, application
                            [{nacho0\cite{Livne2023-bu}, MaterialsBert\cite{Shetty2023-ew}, MatBERT\cite{Trewartha2022-ez}, ChemBERT\cite{Guo2022-kr}, PubMedBERT\cite{Gu2021-yn},  BioMegatron\cite{Shin2020-cp}, BioBERT\cite{Lee2020-vl}, SciBERT\cite{Beltagy2019-ri}, BlueBERT\cite{Peng2019-yb}, etc}, study]
                        ]
                    ]
                    [Mol2Text, task
                        [Molecule captioning, application
                            [{BioT5+\cite{Pei2024-ph}, BioT5\cite{Pei2023-bp}, Text+Chem T5\cite{Christofidellis2023-ea}, Galactica\cite{Taylor2022-pu}, MolT5\cite{Edwards2022-yu}, etc.}, study]
                        ]
                    ]
                    [Mol2Mol, task
                        [Molecule tuning, application
                            [{nacho0\cite{Livne2023-bu}, Regression Transformer\cite{Born2023-nc}, ChemFormer\cite{irwin_chemformer_2022}, etc.}, study]
                        ]
                        [Synthesis prediction, application
                            [{ReactionT5\cite{Sagawa2023-fa},
                            Galactica\cite{Taylor2022-pu}, ChemFormer\cite{irwin_chemformer_2022}, T5Chem\cite{Lu2022-ms}, etc.}, study]
                        ]
                        [Retrosynthesis, application
                            [{Text+Chem T5\cite{Christofidellis2023-ea}, T5Chem\cite{Lu2022-ms}, etc.}, study]
                        ]
                    ]
                    [Mol2Number, task
                        [Property prediction, application
                            [{nacho0\cite{Livne2023-bu}, Regression Transformer\cite{Born2023-nc}, CatBERTa\cite{ock_catalyst_2023}, Darwin\cite{Xie2023-nh}, SELFormer\cite{Yuksel2023-iy}, Galactica\cite{Taylor2022-pu}, ChemBERTa-2\cite{ahmad_chemberta-2_2022}, MolFormer\cite{Ross2022-xf}, Mol-BERT\cite{Li2021-xw}, MTL-BERT\cite{jia_all--one_2021}, ChemBERTa\cite{Chithrananda2020-cd},                             MolBERT\cite{Fabian2020-zd}, SMILES-BERT\cite{wang_smiles-bert_2019}, SMILES transformer\cite{Honda2019-ek}etc}, study]
                        ]
                    ]
                ]
        \end{forest}
    \end{adjustbox} 
    \caption{Classification of LLMs in chemistry and biochemistry according to their application. }
    \label{fig:applications}
\end{figure*}

==> latexdiff.tex <==
\RequirePackage{shellesc}
\ShellEscape{latexdiff main_old.tex main.tex --flatten --debug > main-d.tex}
\input{main-d}

==> paper_old.tex <==
\tableofcontents

\section{Introduction}

The integration of Machine Learning (ML) and Artificial Intelligence (AI) into chemistry has spanned several decades\cite{willett2011chemoinformatics, griffen_chemists_2020, baum_artificial_2021, ayres_taking_2021, yang_concepts_2019, mater2019deep, shi2023machine, keith2021combining, kuntz2022machine, meuwly2021machine}. Although applications of computational methods in quantum chemistry and molecular modeling from the 1950s-1970s were not considered AI, they laid the groundwork. Subsequently in the 1980s expert systems like DENDRAL\cite{lederberg1969applications, lindsay1993dendral} were expanded to infer molecular structures from mass spectrometry data.\cite{buchanan_applications_1976} At the same time, Quantitative Structure-Activity Relationship (QSAR) Models were developed\cite{yang_concepts_2019} that would use statistical methods to predict the effects of chemical structure on activity.\cite{hansch1962correlation, hansch1964p, hansch1995exploring, topliss1972chance} In the 1990s, neural networks were introduced to domains such as drug design, as summarized well by \citet{yang_concepts_2019} and \citet{goldman2006machine}, although they were limited by the computational resources of the time. With an explosion of data from High-Throughput Screening (HTS)\cite{pereira2007origin, medina-franco_shifting_2013}, models then started to benefit from vast datasets of molecular structures and their biological activities. Furthermore, ML algorithms such as Support Vector Machines and Random Forests became popular for classification and regression tasks in cheminformatics,\cite{willett2011chemoinformatics} offering improved performance over traditional statistical methods.\cite{butler_machine_2018}

Deep learning transformed the landscape of ML in chemistry and materials science in the 2010s.\cite{rupp_fast_2012} Recurrent Neural Networks (RNNs),\cite{Olivecrona2017-is, Segler2018-ef, segler_generating_2018, Gupta2018-pj, Karpov2020-yf} Convolutional Neural Networks (CNNs)\cite{schutt_schnet_2018, Hirohara2018-wx, Coley2019-it} and later, Graph Neural Networks (GNNs),\cite{dwivedi2023benchmarking, sanchez2021gentle, bronstein2017geometric, wu2020comprehensive, gilmer2017neural, gomez-bombarelli_automatic_2018} made great gains in their application to molecular property prediction, drug discovery,\cite{gaudelet2021utilizing} and synthesis prediction.\cite{choudhary_recent_2022} Such methods were able to capture complex patterns in data, and therefore enabled the identification of novel materials for high-impact needs such as energy storage and conversion. 
In this review, we explore the next phase of AI in chemistry, namely the use of Large Language Models (LLMs) and Autonomous agents. Inspired by successes in natural language processing (NLP), LLMs like ChemBERTa\cite{Chithrananda2020-cd}, MolBERT\cite{li_mol-bert_2021} and cMolGPT\cite{Wang2023-jd} were adapted for chemical language (e.g., SMILES) to tackle tasks from synthesis prediction to molecule generation. We will then explore the integration of LLMs into Autonomous Agents as illustrated by \citet{Bran2023-jk} and \citet{Boiko2023-ot}, which may be used for data interpretation or, for example, to experiment with robotic systems. We are at a crossroads where the use of AI not only enables chemists to more quickly solve the world's largest problems, but it facilitates the more routine laboratory tasks, which both systematizes the building of larger experimental datasets, and reduces the the lead time for scale up and commercialization of drugs and materials. As such, language has been the preferred mechanism for describing and disseminating research results and protocols for hundreds of years in chemistry. 
The emergence of LLMs enable artificial systems to have the same primary medium as human chemists, facilitating a seamless integration into the scientific workflow.\cite{Vaswani2017-kq, lin_evolutionary_2023, liu_swin_2021, thirunavukarasu_large_2023, khurana_natural_2023} 

% \subsection{Language and chemical language}
% We will define natural language here as the set of default communication syntax with which human beings communicate. That set would include communication in written or audio/oral forms in English, Spanish, Hungarian, Mandarin etc. We refer to the written form of natural language as text. Natural language text is made up of i) letters, ii) subwords, iii) words, iv) sentences, v) paragraphs and vi) essays. Subwords here refer to verb stems and endings, prefixes and suffixes, and sentences will include any combination of subjects, verbs, object, adjective, conjunction etc.
% We then define chemical language as the set of syntax used to communicate the formula, or structure, of a chemical material as a complex combinations of atoms in the periodic table. Since LLMs were built initially for natural language, it is often important to consider the analogies between natural language and chemical language. For example, a Simplified Molecular Input Line Entry System (SMILES) string includes a series of letters with each one representing an atom from the periodic table of elements. We may consider a similar hierarchy that parallels the growth from letters to an essay in natural language, which is described as i) atoms, ii) functional groups, iii) fragments, iv) branches, v) molecules and vi) ensembles. A carbon connected to a terminal oxygen with a double bond is described as the carbonyl functional group, and a collection of squaraine molecules,\cite{wiegand_directional_2024} each with two branches off an aniline fragment may be considered a crystal,\cite{zheng_measurement_2020} or in our terms, an ensemble. It therefore makes sense to recognize that the same types of relationship between, for example, subjects, verbs, sentences and paragraphs also exist in chemical language, where here the paragraph is a molecule. The relationships are of course different but the LLM can learn these relationships in exactly the same way as it learns natural language patterns, which of course it has no prior knowledge of before the pretraining.
% Nevertheless we refer to natural language pre-trained transformers as Text-LLMs and chemical language pre-trained transformers as Mol-LLMs. We thereby follow the convention introduced by Zhang et al.\cite{Zhang2024-na}

\subsection{Challenges in chemistry}

With the potential to accelerate progress through the use of AI, and in particular LLMs, it makes sense to connect this potential to some of the more pressing opportunities in the chemical sciences as may be categorized under three broad umbrellas: Property Prediction, Property Directed Molecule Generation and Synthesis Prediction. 
The First challenge is to predict a property for a given compound to decide if it should be synthesized for a specific application, such as an indicator,\cite{collison_complexation_2008} light harvester,\cite{wiegand_directional_2024} or catalyst.\cite{ahmadov_dual_2024} To have better models for property prediction, good quality data is crucial. We discuss the caveats and issues with the current datasets in Section \ref{sec:benchmark} and illustrate state-of-the-art findings in Section \ref{sec:sciEncoder}
% While it is possible to calculate expected properties from a chemical structure, the goal is to significantly reduce computational resources needed, such as for predicting condensed phase properties using physics-based molecular dynamics or quantum calculations.\cite{pablo-garcia_fast_2023}

The second challenge is to generate novel chemical structures that meet desired chemical profiles or specific properties.\cite{fischer_approaching_2019} Success would accelerate progress in various chemical applications, but reliable reverse engineering (inverse design)\cite{wang_data-driven_2022} is not yet feasible over the vast chemical space.\cite{sridharan_modern_2022} For instance, inverse design coupled with automatic selection of novel structures (\textit{de novo} molecular design) could develop a drug targeting a specific protein while retaining properties like solubility, toxicity, and blood-brain barrier permeability.\cite{wu_moleculenet_2018} The complexity of connecting \textit{de novo} design with property prediction is high and raises ethical questions that need to be addressed to guide the development of such models. We show how state-of-the-art models currently perform in Section \ref{sec:SciDecoder}. 

% The second challenge would be to generate novel chemical structures that might satisfy some desired chemical profile or a particular set of needed properties.\cite{fischer_approaching_2019} Success here would greatly accelerate progress in a variety of chemical applications, but this kind of reverse engineering (or inverse design)\cite{wang_data-driven_2022} cannot currently be done with any reliability over an almost infinite chemical space\cite{sridharan_modern_2022}. To illustrate inverse design coupled with the automatic selection of novel chemical structures (``\textit{de novo} molecular design''), a drug might be developed specifically to be active towards a particular target protein. The molecule may also be tailored to retain additional drug-like properties beyond target-binding efficacy, such as solubility, toxicity and the ability to cross the blood-brain barrier, to name a few.\cite{wu_moleculenet_2018} The complexity associated with this connection of \textit{de novo} design and property prediction is high.

The third major challenge is predicting its optimal synthesis using inexpensive, readily available, and non-toxic starting materials. There will always likely be a solution within a large chemical space: an alternative molecule with similar properties that is easier to synthesize. Exploring this space to find a new molecule with the right properties and a high-yield synthesis route unites these challenges. The number of possible stable chemicals is estimated to be up to $10^{180}$.\cite{restrepo_chemical_2022, kirkpatrick2004chemical, mullard2017drug, llanos2019exploration} Exploring this vast space requires significant acceleration beyond current methods.\cite{schrier_pursuit_2023} \citet{restrepo_chemical_2022} emphasizes the need to catalog data on failed syntheses to build a comprehensive dataset of chemical features. Autonomous chemical resources can accelerate database growth and tackle this challenge. Thus, automation is considered a fourth major challenge in chemistry.\cite{gromski2019explore, steiner2019organic, burger2020mobile, macleod2020self} The following discussion explores how Large Language Models (LLMs) and Autonomous Agents can provide the most value. Relevant papers are discussed in Section \ref{sec:sciEncDec}

% Even once a molecule is prescribed, the third major challenge would be to predict the optimal synthesis (including yield) of that molecule of interest. This challenge also includes the ability to work from starting materials that are inexpensive, readily available and non-toxic. Thankfully, there is likely to always be a possible solution; in a large chemical space, a different molecule will likely exist with similar specific properties required for the target application, yet a molecule that can be more easily synthesized (versus other candidates). Being able to explore a large chemical space, to identify a new and valid molecule that can be predicted to have the right properties and be readily synthesized against a predicted high-yield route, is the task that unites these three challenges. Estimates of the number of possible chemically and physically stable chemicals is up to $10^{180}$.\cite{restrepo_chemical_2022, kirkpatrick2004chemical, mullard2017drug, llanos2019exploration} Exploring that entire chemical space is a daunting task, necessitating significant acceleration beyond current methods.\cite{schrier_pursuit_2023} \citet{restrepo_chemical_2022} highlights the critical need to catalog data even on failed syntheses to build a more comprehensive dataset of chemical features\cite{restrepo_chemical_2022}. The ability to dedicate autonomous chemical resources to accelerate growth in our databases may allow us to tackle this challenge. We therefore consider a fourth large umbrella of challenge in chemistry to be automation.\cite{gromski2019explore, steiner2019organic, burger2020mobile, macleod2020self} With these being the largest challenges in chemistry we continue below to discuss where Large Language Models (LLMs) and Autonomous Agents can provide the most value. 

Here, we provide a comprehensive review of large language models and autonomous agents within the context of these chemical challenges. We identify gaps between current capabilities and future progress in chemistry that AI can bridge. 
% While human expertise still leads progress in the areas of property prediction, property-directed molecular design, and synthesis prediction, automation presents the greatest opportunity for acceleration through the revolution in autonomous agents that is upon us. Hence, we are well positioned to navigate through that vast chemical space. 
The structure of the review is as follows. Section 2 provides an introduction to transformers, including a brief description of encoder-only, decoder-only and encoder-decoder architectures. Section 3 provides a detailed survey of work with LLMs, where we connect each transformer architecture to the areas of chemistry that it is best suited to support. We then progress into a description of autonomous agents in section 4, and a survey of how such LLM-based agents are finding application in chemistry-centered scientific research, section 5. After providing some perspective on future challenges and opportunities in section 6, and we conclude in section 7. 
Throughout the following, we separate our descriptions based on "text-based" inputs and outputs along with "mol-based" inputs and outputs, following a similar convention introduced by Zhang et al.\cite{Zhang2024-na}. We therefore define "text" as natural language, the set of default communication syntax with which human beings communicate. We then define "mol" as the set of syntax used to communicate the formula, or structure, of a chemical material as a complex combination of atoms in the periodic table, commonly using a string representation. 
% By default we use the Simplified Molecular Input Line Entry System (SMILES) string to represent chemical language, recognizing that chemical properties change significantly\cite{wiegand_directional_2024, zheng_measurement_2020} as we move from atoms, functional groups, molecules to molecular ensembles, or crystals. This mirrors the way that meaning changes as we move from individual words to collections of paragraphs. 

\section{Large Language Models}

Large Language Models (LLMs) are deep neural networks (NN) with billions of parameters. Mostly, LLMs implement a transformers architecture, introduced by \citet{Vaswani2017-kq}, although other architectures for longer input sequences\footnote{These longer sequences are more important in biology, where whole genomes are pursued} are being actively explored\cite{Gu2023-gp,Jelassi2024-dj,peng2023rwkv}. Transformers are well-developed in chemistry and are the dominant paradigm behind nearly all state-of-the-art results and, thus, the focus.

%Mamba's time complexity scales linearly ($O(n)$) while transformers scale quadratically ($O(n^2)$), which may be a problem for very long sentences. Despite being memory efficient and faster during inference time, SSSMs may suffer memory loss due to tasks that require copying from the context.\cite{Jelassi2024-dj}
%In addition, transformers have a very well-developed community and ecosystem.  herefore, the fulcrum of this review is the transformer network architecture.

\subsection{The Transformer}

\begin{figure}[h!]
    \centering
    \includegraphics[width=1.0\textwidth]{figs/transformer_all_combined.png}
    % \includegraphics[width=0.37\textwidth]{figs/encoder_decoder_modified_5_24_24.png}    \includegraphics[width=0.60\textwidth]{figs/transformers_in_chemistry_combined_v2.png}
    \caption{a) The generalized encoder-decoder transformer: The encoder on the left converts an input into a vector, while the decoder on the right predicts the next token in a sequence. b) Encoder-decoder transformers are traditionally used for translation tasks and, in chemistry, for reaction prediction, translating reactants into products. c) Encoder-only transformers provide a vector output and are typically used for sentiment analysis. In chemistry, they are used for property prediction or classification tasks. d) Decoder-only transformers generate likely next tokens in a sequence. In chemistry, they are used to generate new molecules given an instruction and description of molecules.
    % extrapolate to modified or larger molecules from a set of input molecules.
    }
    \label{fig:transformer}
\end{figure}

The transformer was introduced in, ``Attention is all you need'' by \citet{Vaswani2017-kq} in 2017. A careful line-by-line review of the model can be found in ``The Annotated Transformer'' \cite{annotated_transformer}. The transformer was the first sequence-to-sequence (seq2seq) model based entirely on attention. Here, a seq2seq model processes a text input, such as an English paragraph, and produces a different text sequence, such as a French translation of that paragraph. The concept of ``attention'' is a focus applied to certain words of the input, which would convey the most importance, or the context of the passage, and thereby would allow for better decision-making and greater accuracy. However, in a practical sense, ``attention'' is implemented simply as the dot-product between token embeddings with some non-linear learned function, and is described further below.

The prior state-of-the-art for seq2seq was considered to be the Recurrent Neural Network (RNN),\cite{rumelhart1986learning} typically as implemented in \citet{hochreiter1997long}. The RNN retains ``memory'' of previous steps in a sequence to predict later parts. However, as sequence length increases, gradients can become vanishingly small or explosively large\cite{ribeiro_beyond_2020, or_exploding_2023}, preventing effective use of earlier information in long sequences. RNNs have thus fallen behind transformers, but recent progress has seemed to enable comparable models to transformers\cite{Gu2023-gp, peng2023rwkv}.

% Furthermore, since the RNNs worked fundamentally with a series of steps in the sequence, then they would not parallelize so well, which limits their ability to take advantage of Graphical Processing Units (GPUs).
The transformer architecture implements two main modules: the encoder and the decoder. Figure \ref{fig:transformer}a provides a cartoon diagram of the general encoder-decoder transformer architecture.
%The decoder stack passes an input position-encoded embedding to a masked multi-head attention layer, whose job is to predict the next word in the sequence, which is only possible after those latter words in the sequence have been masked from the decoder's view. (The Transformer model in the original paper uses a sequence-to-sequence approach where the decoder generates the output sequence one token at a time, conditioned on the encoded input and what it has generated so far). Since the resulting linear vector from the encoder stack is also passed to a multi-attention head in the decoder stack, that decoder stack is now connected to the encoder since it can thus peek back at the so-called latent vector. The decoder gradually builds up combinations to get iteratively better responses.
The input is first tokenized, from the model's vocabulary,\cite{Kudo2018-bf, Kudo2018-aq, Song2020-lo, Rust2020-vs, Berglund2023-nz}  into computable integers that are then converted into numerical vectors using embedding layers in the bottom most encoder. A single encoder stack is shown here, where in reality there are many, with six in the original model.\cite{Vaswani2017-kq} The later stacks each use outputs from the prior stack, typically as a $\sim$512 per-token vector.
Each encoder applies positional encoding typically using sine and cosine functions, with a frequency depending on that word's position, to handle sequences of any length. Other functions can also be used.\cite{Gehring2017-zj} The encoder stack then comprises a multi-headed self-attention mechanism, which relates each “word” to others in the sequence by computing attention scores based on queries, keys, and values. This is followed by normalization and residual connections. Residual connection is represented in Figure 1a by the “by-passing” arrows, which indicate how each sub-layer output is added to its input, which helps mitigate the vanishing gradient problem.\cite{ribeiro_beyond_2020, or_exploding_2023} Lastly, the output is further refined through a pointwise feed-forward network with ReLU activation, resulting in a set of vectors representing the input sequence with rich contextual understanding, ready for the decoder.


Similarly, the decoder workflow begins with converting the initial input token into numerical vectors, known as the output embedding step, as this initial input serves as the start token for the model's final output. Positional encodings are then added, followed by a stack of approximately six identical decoder layers. Each decoder layer includes a Masked Self-Attention Mechanism to prevent positions from attending to subsequent ones and an Encoder-Decoder Multi-Head Attention to align encoder outputs with decoder attention layer outputs (indicated by the square connecting arrows in Figure \ref{fig:transformer}a), focusing on relevant parts of the input. A fully connected Feed-Forward Neural Network refines the output further. The final layer acts as a linear classifier, mapping the output to the vocabulary size, and a softmax layer converts this output into probabilities, with the highest indicating the predicted next word. Each sub-layer is followed by normalization and includes a residual connection. The decoder generates output sequences autoregressively, incorporating each newly predicted token until an end token signals completion.
Figure \ref{fig:transformer}b shows a cartoon illustration of the encoder-decoder model’s strength in translating between languages or from atoms in reactants mapped into new positions in associated products. Figure \ref{fig:transformer}c depicts the ability of an encoder-only model to detect an additional meaning, or property, from an input sequence, represented as a number description. Figure \ref{fig:transformer}d presents a cartoon depiction of a decoder-only architecture inferring and generating a consequence, based on an original input. Hence, a new peptide sequence has been inferred after the combined input of two smaller amino acids, indicating how the decoder-only approach can be used to generate potentially new compounds. 

%\paragraph{Tokenization} The user inputs a natural language text into the model. In NLP tasks, the sequence is then converted to a list of tokens, which are computable integers each indicating a sequence fragment indexed in the model's vocabulary. The sentence is converted to tokens following a specific tokenization scheme.\cite{Kudo2018-bf, Kudo2018-aq, Song2020-lo, Rust2020-vs, Berglund2023-nz}
%The user inputs a natural language text into the model. However, that's not the representation used by the LLM to make computations. In NLP tasks, the sequence is converted to a list of tokens -- integers indicating sequence fragments according to the model's vocabulary. The sentence is converted to tokens following a specific tokenization scheme.\cite{Kudo2018-bf, Kudo2018-aq, Song2020-lo, Rust2020-vs, Berglund2023-nz}
%\paragraph{Input Embeddings} Input embeddings are responsible for converting the discrete sequence input (list of tokens) into a more compact continuous space. Each token is substituted for a vector of continuous values. The input embedding returns a learned representation for each token that focuses on adding semantic meaning to similar tokens.

%\paragraph{Positional encoding} Positional encoding plays a major role in transformer success. It is added to the input embeddings to provide information about the sequence order. Many choices for positional embeddings are available.\cite{Gehring2017-zj} \citet{Vaswani2017-kq} reported equivalent results with both fixed positional encoding using sine and cosine functions and learned encoding.
%The positional encoding occurs for words in a sentence by adding some second number to an original number that was associated with the meaning of the word through ``embedding'' and after ``tokenization''. The combination of a positional number to the original embedding forms a now-modified vector. Cosine and sine functions of different frequencies (based on the position of the word in the sequence) would ensure that the positional encoding would be unique to that word's position, independent of the length of the sequence. Moreover, the cosine or sine function would provide manageable values between -1 and 1.

%\paragraph{Positional encoding} Positional encoding plays a major role in transformer success. It is added to the input embeddings to provide sequence order information and there are various positional embedding methods.\cite{Gehring2017-zj} For example, cosine and sine functions of different frequencies (based on the position of the word in the sequence) would ensure that the positional encoding would be unique to that word's position, independent of the length of the sequence. Here, the cosine or sine function would provide manageable values between -1 and 1.\citet{Vaswani2017-kq} reported equivalent results with both fixed positional encoding using sine and cosine functions and learned encoding. 


%\paragraph{Attention} Attention is a mechanism that enables the model to focus on specific parts of the input data. After positional encoding the ``attention'' between every pair of words in a sequence can be computed. 
%Each word may be considered a ``query'' and is compared to every other word, or ``key'', with each key having its own ``value''. Similarities (or connections) between query and key would lead to the associated value being multiplied by a weighted ``attention''. 
%Hence, when words are connected to other words in a sequence, that connection is weighted higher. With multiple passes through the attention head, pairs of pairs, and then pairs of pairs of pairs etc. can be connected such that a meaning is embedded to a final linear output, which would then be passed to the output.

% \subsubsection{Attention}

% Attention enables the model to focus on specific parts of the input data. After positional encoding, attention between word pairs in a sequence is computed. Thus, each word or "query" is compared to every other word, or "key". Each word also has a "value", and the similarity between query and key results in a weighted attention applied to that value. Multiple passes through the attention head connect word pairs, embedding meaning into the final output.

% In other words, ``attention'' is a scaled dot-product operation, a mathematical mechanism that has three matrices with trainable weights (referred to as $q$, $k$, and $v$) that are multiplied with the input to generate the query ($Q$), key ($K$), and value ($V$) matrices. The generated scores weight the relevance of other keys when processing a given query, thereby allowing the model to dynamically focus on the most relevant parts of the input sequence.
% The output of the attention layer is computed by:

% \begin{equation}
%     Attention(Q,K,V) = softmax\left( \frac{QK^{T}}{\sqrt{d_k}}\right)V
% \end{equation}

% where $d_k$ is a hyperparameter, often assumed to be equal to the key's dimension, giving the name `scaled'. The right-hand side of this equation is composed of two terms, the first term has a softmax function and is trained to be non-zero in positions relevant to processing a given position in the $V$ matrix. A multi-head attention is a concatenation of $h$ attention operations. Each attention has its own set ($q$, $k$, $v$). It enables the model to tune its parameters to focus on information on different parts of the representation.


% Attention is a mathematical operation. \citet{Vaswani2017-kq} implemented scaled dot-product attention with three trainable matrices ($q$, $k$, $v$), generating query ($Q$), key ($K$), and value ($V$) matrices. The scores weight the relevance of the key when processing a query, allowing dynamic focus on input sequence parts. The attention layer output is:

% \begin{equation}
% Attention(Q,K,V) = softmax\left( \frac{QK^{T}}{\sqrt{d_k}}\right)V
% \end{equation}

% where $d_k$ is a hyperparameter, typically equal to the key's dimension. Multi-head attention concatenates $h$ attention operations, each with its set ($q$, $k$, $v$), enabling the model to focus on different representation parts.
%\paragraph{Encoder}The encoder is responsible for processing the sequence such that an optimized learned representation is output. This output is also known as the features. From the architecture point of view, the encoder is built by a stack of $N$ identical layers, where each layer implements a multi-head attention, followed by a fully connected feed-forward network. The encoder processes the entire sequence and is suitable for tasks that require a global bi-directional understanding of the sequence, such as sentence classification, named entity recognition (NER), and question-answering (QA).

%\paragraph{Decoder}The decoder uses the features together with another input sequence to generate the translated output sequence. Its architecture is very similar to the encoder. It also has $N$ stacked identical layers; however, it adds one more multi-head attention operation over the features. Therefore, each decoder stack has a first multi-head attention layer, which processes the decoder's input, a second multi-head attention that together processes the output of the encoder stack along with the output of the decoder's first multi-head attention layer and, finally, a fully connected feed-forward network. Decoders work auto-regressively, meaning they predict the completion of the sequence at position $i$ using information from positions less than $i$. Decoders are therefore suitable for generative tasks such as the next word completion.

%\paragraph{Parallelization}The Transformer uses ``multiple attention heads'' to allow the model to attend to different parts of the sequence in parallel. The benefit here is that the model can capture additional aspects of the sequence, such as different types of syntactic and semantic relationships, simultaneously. Furthermore, the transformer also applies additional layers, such as feed-forward neural networks (FFNN) and normalization layers. FFNN add necessary non-linearities to the model since, otherwise, the entire system would be reduced to a single linear output and the complexity would be lost. Normalization reduces the number of steps required in gradient descent optimization and also reduces training problems originating from the necessary layer interdependencies.

\subsection{Model training}

The common lifetime of an LLM consists of being first pre-trained using unsupervised or self-supervised techniques, generating what is called a base model.
This base model is then fine-tuned for specific applications using supervised techniques. Finally, the supervised fine-tuned model is further tuned with reward models to improve human preference or some other non-differentiable and sparse desired character\cite{stiennon2020learning}.
%However, supervised fine-tuning might not be enough to align the model accordingly to the expected generation at some times. Lack of a good alignment could cause the model to respond unsafely -- either with offenses or, in natural science models, potentially enabling dual usage. 
%Reinforcement learning (RL) allows us to control the tone and address safety issues regarding dual-use by interactive fine-tuning.
%This process is interestingly illustrated by \texttt{@anthrupad} in a tweet.\cite{anthrupad2023-xd}

\paragraph{Unsupervised pretraining}

A significant benefit implied in all the transformer models described in this review is that unsupervised learning takes place with a vast corpus of text. Thus, the algorithm learns patterns from untagged data, which opens up the model to larger datasets that may not have been explicitly annotated by humans. The advantage is to discover underlying structures or distributions without being provided with explicit instructions on what to predict, nor with labels that might indicate the correct answer.
% Thus the first stage of learning for GPT involves predicting the next word in a sequence given the previous words in that sequence.

\paragraph{Supervised fine-tuning} After this pretraining, many models described herein are fine-tuned on specific downstream tasks (e.g., text classification, question answering) using supervised learning. In supervised learning, models learn from labeled data, and map inputs to known outputs. Such fine-tuning allows the model to be adjusted with a smaller, task-specific dataset to perform well on that downstream task.

\paragraph{Reinforcement learning}
A key task after model training is to align its output with what human users prefer. This can only be evaluated on complete outputs from models, preventing supervised fine-tuning (which requires token-by-token data). Thus reinforcement learning is used for these sparse signals.
Reinforcement Learning (RL) is a type of machine learning where actions are performed and feedback is received through rewards, the goal being to learn a policy that maximizes the cumulative reward.\cite{Duan2016-qs}
To apply RL, sampling tokens from the model is recast as a Markov Decision Process (MDP).\cite{Laskin2022-cn}
A MDP is defined by state $S$ -- a set of states ${s}$, the action space $A$ -- a set of possible actions ${a}$, the transition dynamics $P(s'|s, a)$ -- a probability density function to model the probability of the new state given the current state and the action used, and a reward function $r(s', s)$ -- the signal to improve the model.\cite{Mazuz2023-gb}
The LLM is a policy in this setting: a way to map from $s$ to $a$ that maximizes the cumulative reward, which concludes at the end of the LLMs completion\cite{Ziegler2019-da}.
The most known application is reinforcement learning from human feedback (RLHF), which consists of three steps: ($1$) Given the dataset, multiple policies are used to sample a set of model completions, which are judged by a human. Then, ($2$) a reward model -- usually another LLM -- is trained to reproduce human feedback. Finally, ($3$) a policy gradient method such as proximal policy optimization (PPO)\cite{Schulman2017-lw} or REINFORCE\cite{Zhang2020-ji} is used to optimize the policy.\cite{Stiennon2020-kk}
Alternatives to RLHF have been proposed.\cite{Duan2016-qs, Laskin2022-cn, Shinn2023-kt, Akyurek2023-ms, Rafailov2023-hc}
A general discussion about RL potential for LLM fine-tuning was published by \citet{Cao2024-yf}.

% In other words, the idea was to leverage large-scale unsupervised pretraining followed by supervised fine-tuning to achieve state-of-the-art performance for a broader range of natural language processing (NLP) tasks. We will later find that the use of LLMs in tackling chemistry problems will almost universely rely on the ability to learn patterns from large unlabeled chemical datasets, which provides significant potential for accelerating progress in AI for chemistry application.

% ``Teacher forcing'' is a training strategy used in sequence-to-sequence models where the true output sequence up to the current token is used as input to the decoder stack during training, rather than the model's own predictions. When testing the model, individual words can be added one by one to the encoder stack of the model such that the accuracy of the translation can be determined.

% Above all, the transformer architecture was a pioneering next step since state of the art accuracies could be attained with orders of magnitude reductions in computational times, largely through parallization. The Vaswani architecture builds an understanding of the input such that the understanding can be translated into the same understanding but in a different language.

\subsection{Model types}

% LLaMA, LLaMA2, Vicuna, Galactica, Smaug, Chinchilla, Gopher, Claude, Megatron, Codex, PaLM, PaLM-E, PaLM2, Gemini, Alpaca, Giraffe, Mistral, VoxtLM, Zephyr,

While the Vaswani Transformer\cite{Vaswani2017-kq} employed an encoder-decoder structure for sequence-to-sequence tasks, the encoder and decoder were ultimately seen as independent models, leading to ``encoder-only'', and ``decoder-only” models described below.
%that interact to create the transformers. However, some studies were made investigating the capabilities of encoders and decoders separately. An LLM that uses only the encoder part of the transformer is called an ``encoder-only model''. Analogously, an LLM that has only the decoder is called a ``decoder-only model''.

\subsubsection{Encoder-only models}

Beyond Vaswani's transformer,\cite{Vaswani2017-kq} used for sequence-to-sequence tasks, another significant evolutionary step forward came in the guise of the Bidirectional Encoder Representations from Transformers, or ``BERT'', described in October 2018 by \citet{Devlin2018-nl}
%BERT utilized only the encoder component, achieving as-of-then state-of-the-art performance on sentence-level and token-level (word-level) tasks, while outperforming some prior task-specific architectures.\cite{Devlin2018-nl} While the encoder architecture was the same for both Vaswani,  and Devlin, it was the bidirectional transformer pretraining on unlabeled text that made the difference. By ``bidirectional'', this means that the model looks at the context both to the left and to the right of the word in question facilitated by a Masked Language Model (MLM). This allows a richer understanding of the meaning of the sentence. The encoder-only design choice would mean that BERT would focus on generating a much deeper ``understanding'' of the input sequence, rather than mapping input sequences to output sequences. A ``sequence'' is an input token sequence, which may be made up of one or more of such sentences.
BERT utilized only the encoder component, achieving state-of-the-art performance on sentence-level and token-level tasks, outperforming prior task-specific architectures.\cite{Devlin2018-nl} The key difference was BERT's bidirectional transformer pretraining on unlabeled text, meaning the model looks at the context both to the left and right of the word in question, facilitated by a Masked Language Model (MLM). This allows a richer understanding of the sentence. The encoder-only design meant BERT focused on generating a deeper "understanding" of the input sequence, rather than mapping input sequences to output sequences.
%In pretraining, BERT uses a Masked Language Model (MLM) and Next Sentence Prediction (NSP). We note that ``sentence'' here means an arbitrary span of contiguous text, which may not be an actual grammatical sentence. The MLM task will randomly mask tokens in that sentence and then predict these masked tokens by looking at both the preceding words and context, and the following words and context, simultaneously. (The MLM approach was inspired by Taylor\cite{taylor_cloze_1953}). NSP involves predicting whether one sentence logically follows another, training the model to understand the relationship between sentences.  Ultimately, the simultaneous bidirectional approach allows BERT to recognize greater nuance and richness in the input data.
In pretraining, BERT also uses Next Sentence Prediction (NSP). "Sentence" here means an arbitrary span of contiguous text. The MLM task randomly masks tokens and predicts them by looking at preceding and following contexts simultaneously, inspired by Taylor\cite{taylor_cloze_1953}. NSP predicts whether one sentence logically follows another, training the model to understand sentence relationships. This bidirectional approach allows BERT to recognize greater nuance and richness in the input data.

%There have been many subsequent evolutions of BERT, including RoBERTa (Robustly optimized BERT approach) from 2019 described by Facebook AI's \citet{liu_roberta_2019} RoBERTa was trained on a much larger corpus of text compared to BERT, which improved the model's understanding and generalization capabilities. RoBERTa was also trained for more iterations, with larger mini-batches and longer sequences, which allowed the model to learn more complex patterns and relationships in the data. By removing the NSP task and simply training the model more extensively on the masked language model (MLM) task, better performance was also achieved. Unlike BERT, which pre-determined the masked tokens in the pre-processing step, RoBERTa dynamically changed the masked positions during the training process thereby exposing the model to a more diverse set of patterns. Lastly, RoBERTa used different hyperparameters, such as learning rates and batch sizes, another evolution beyond BERT. Evolutions of BERT also include pretraining with domain-specific data, creating a specialist LLM (see Section \ref{sec:LLM_in_science}), and we further describe below the use of BERT in chemical-language- and natural-language-based LLMs, addressing several challenges in chemistry.

Subsequent evolutions of BERT include, for example, RoBERTa, (Robustly optimized BERT approach), described in 2019 by Facebook AI's \citet{liu_roberta_2019}. RoBERTa was trained on a larger corpus, for more iterations, with larger mini-batches, and longer sequences, improving model understanding and generalization. By removing the NSP task and focusing on the MLM task, performance improved. RoBERTa dynamically changed masked positions during training and used different hyperparameters. Evolutions of BERT also include domain-specific pretraining, creating specialist LLMs for fields like chemistry, as described below (see Section \ref{sec:LLM_in_science}).

\subsubsection{Decoder-only models}

%In June 2018, \citet{radford_improving_nodate} from OpenAI proposed the Generative Pretrained Transformer (GPT) in their paper, ``Improving Language Understanding by Generative Pretraining''. Essentially, they had followed up with a decoder-only system, which departed from sequence-to-sequence tasks in favor of left-to-right unidirectional language modeling. GPT was pre-trained to predict the next word in a sequence based on the previous words, and it used only the decoder part of the Transformer architecture. There were no encoded representations from an encoder so it was not well set up to obtain an understanding of the input. However, unlike the Vaswani Transformer's decoder, it could predict the likely next sequence. In other words, whereas the end-to-end Vaswani transformer would only allow a translation of the original meaning into a different ``language'', GPT could be predictive of a consequence, given the prior text, and the supervised fine-tuning. This powerfully enabled GPT to apply its general language understanding towards specific tasks, when only smaller annotated datasets were available.
%
%As with the Vaswani Transformer, GPT employed positional encodings to maintain the order of words in its predictions. These encodings ensured that despite the parallel processing capabilities of the Transformer architecture, the model could still comprehend and generate sequences where the order of tokens is crucial. However a nuanced difference was with the masked attention. In the GPT architecture, the self-attention mechanism was adapted to prevent each token from attending to future tokens in the sequence; the prediction of each word would depend only on the words that came before it.

In June 2018, \citet{radford2018improving} from OpenAI proposed the Generative Pretrained Transformer (GPT) in their paper, "Improving Language Understanding by Generative Pretraining". GPT used a decoder-only, left-to-right unidirectional language model to predict the next word in a sequence based on previous words, without an encoder. Unlike the Vaswani Transformer's decoder, GPT could predict the next sequence, applying general language understanding to specific tasks with smaller annotated datasets.

GPT employed positional encodings to maintain word order in its predictions. Unlike the Vaswani Transformer, GPT's self-attention mechanism prevented tokens from attending to future tokens, ensuring each word prediction depended only on preceding words.
Hence a decoder-only architecture represents a causal language model, one that generates each item in a sequence based on the previous items; the generation of each subsequent output is causally linked to the history of generated outputs and nothing ahead of the current word affects its generation.

\subsubsection{Encoder-decoder models}

Evolving further, BART (Bidirectional and Auto-Regressive Transformers) was introduced by \citeauthor{lewis_bart_2019} from Facebook AI in 2019.\cite{lewis_bart_2019} BART combined the context learning strengths of the bidirectional BERT, and the autoregressive capabilities of models like GPT, which excel at generating coherent text. BART was thus a hybrid seq2seq model, consisting of a BERT-like bidirectional encoder and a GPT-like autoregressive decoder. BART was pre-trained using a task that corrupted text by, for example, deleting tokens, and shuffling sentences. It then learnt to reconstruct the original text.
%There continues to be advances in LLM development, but we refine our focus below on the use of LLMs to tackle challenges in Chemistry.

\subsubsection{Multi-task and multi-modal models}

% In previous sections, we discussed LLMs whose input may have been one form of text (natural language or chemical language) and whose output was either a learned representation or text in a form similar to the input langauge. In addition to performing a task -- such as text translation, summarization, classification, and so on -- LLMs were developed to accept different tasks using the same weights. \citet{Raffel2019-uy} developed the Text-to-Text Transfer Transformer (T5) to show that different tasks can be cast as text-to-text task. Therefore, the same model architecture and training procedure could be used, disregarding the specific task of interest. T5 motivated research on multi-task models, where the model is able to adapt to different tasks in inference time. For instance, Flan-T5\cite{Chung2022-yp} used instruction fine-tuning to fine-tune the model to respond to different tasks accurately. Flan-T5 is fine-tuned with instructions and chain-of-thoughts prompts, and the authors showed that it could even generalize for unseen tasks, such as instructing the model to generate the rationale before answering. Other more complex approaches have also been suggested for more robust multi-task models.\cite{Tan2023-gt, Shen2024-dh, Son2024-nm, Feng2024-iv}

%In previous sections, we discussed LLMs whose input is usually text using natural language and output either a learned representation or another natural language text. In addition to performing a task -- such as text translation, summarization, classification, and so on -- LLMs were developed to accept different tasks using the same weights. \citet{raffel_exploring_2020} developed the Text-to-Text Transfer Transformer (T5) to show that different tasks can be cast as a text-to-text task. Therefore, the same model architecture and training procedure could be used, disregarding the specific task of interest. T5 motivated research on multi-task models, where the model is able to adapt to different tasks in inference time. For instance, Flan-T5\cite{Chung2022-yp} used instruction fine-tuning to fine-tune the model to respond to different tasks accurately. Flan-T5 is fine-tuned with instructions and chain-of-thoughts prompts, and the authors showed that it could even generalize for unseen tasks, such as instructing the model to generate the rationale before answering. Other more complex approaches have also been suggested for more robust multi-task models.\cite{Tan2023-gt, Shen2024-dh, Son2024-nm, Feng2024-iv}


%Additionally, despite receiving only text, LLMs have been extended to understand different types of input, or ``modalities''. For instance, Fuyu\cite{FUYU8B-2023} uses a linear projection to adapt the encoded representation of images into the tokens space of an LLM. Therefore, a decoder-only model could be trained to write figure captions. Scaling up this concept, next-GPT\cite{Wu2023-pw} was developed as an ``any-to-any'' model, meaning any modality could be input for any task, and any output could be generated. Specifically, multiple modalities -- text, audio, image, and video -- can be processed by a modality-specific encoder and the encoded representation would be projected into a decode-only token space. Then, the output generated by the LLM is processed to separate the generations for each modality, and a domain-specific diffusion model generates each modality output.

In previous sections, we discussed LLMs that take natural language text as input and then they output either a learned representation or another text sequence. These models traditionally perform tasks like translation, summarization, and classification. \citet{Raffel2019-uy} developed the Text-to-Text Transfer Transformer (T5) to demonstrate that various tasks can be reframed as text-to-text tasks, allowing the same model architecture and training procedure to be used with the same set of weights across different tasks. This approach has inspired the development of multi-task models that can adapt to different tasks at inference time. For example, Flan-T5\cite{Chung2022-yp} used instruction fine-tuning with chain-of-thought prompts, enabling it to generalize to unseen tasks, such as generating rationales before answering. More complex approaches have been proposed for robust multi-task models.\cite{Tan2023-gt, Shen2024-dh, Son2024-nm, Feng2024-iv}

Additionally, LLMs have been extended to understand different input modalities, despite initially receiving only text. For instance, Fuyu\cite{FUYU8B-2023} uses linear projection to adapt image representations into the token space of an LLM, enabling a decoder-only model to write figure captions. Scaling up, next-GPT\cite{Wu2023-pw} was developed as an "any-to-any" model, processing multiple modalities—text, audio, image, and video—through modality-specific encoders. The encoded representation is projected into a decoder-only token space, and the LLM's output is processed by a domain-specific diffusion model to generate each modality's output. Multitask or multimodel methods are further described below as these methods start to connect LLMs with the Autonomous Agents.

\section{LLMs for chemistry and biochemistry}\label{sec:LLM_in_science}

\subsection{Molecular Representations, Datasets, and Benchmarks}\label{sec:benchmark}

Given the diversity of data in chemistry-based machine learning, and the many different ways that a compound can be described, from molecular structure to property description, there are multiple ways a molecule can be represented, underlining this heterogeneity.\cite{lo2018machine, david_molecular_2020, Atz2021-nh, Walters2021-ck} Some common forms include molecular graphs\cite{chen2019graph, hu2020open, kearnes2016molecular}, 3D point clouds\cite{wang2022point, thomas2018tensor, wang2021seppcnet, ahmadi2024machine}, and quantitative feature descriptors.\cite{singh_molecular_2023, Bran2023-oi, shilpa_recent_2023, Wigh2022-kf, david_molecular_2020} In this review, We will focus on string-based representations of molecules, given the interest in language models. Among the known string representations, we can cite SMILES,\cite{weininger_smiles_1988} DeepSMILES,\cite{oboyle_deepsmiles_2018} SELFIES,\cite{krenn_self-referencing_2020} and InChI,\cite{heller_inchi_2015} as recently reviewed by \citet{Das2024-ad}.

%Molecules can be depicted through various representations for machine learning applications, as highlighted by several researchers.\cite{david_molecular_2020, Atz2021-nh, Walters2021-ck} Some common forms include molecular graphs, 3D point clouds, and quantitative feature descriptors.\cite{singh_molecular_2023, Bran2023-oi, shilpa_recent_2023, Wigh2022-kf, david_molecular_2020} Given the diversity of data in chemistry-based machine learning, these multiple representations underline the field's heterogeneity.

%However, this review will specifically concentrate on textual representations of molecules, which align with our focus on language models. Prominent string-based representations include SMILES,\cite{weininger_smiles_1988} DeepSMILES,\cite{oboyle_deepsmiles_2018} SELFIES,\cite{krenn_self-referencing_2020} and InChI.\cite{heller_inchi_2015} These have been extensively reviewed and provide a robust framework for our discussions on molecular modeling using language models.

% Large datasets are important for pretraining LLMs. Databases like PubChem, ChEMBL, and ChemSpider are used for pretraining and have also been used for measuring performance.  The connectivity and stereochemistry of molecules may be captured in terms of  and there are ways to convert molecular representations to quantitative features\cite{singh_molecular_2023, Bran2023-oi, shilpa_recent_2023, Wigh2022-kf, david_molecular_2020}. 

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.6\textwidth]{figs/token_dist.pdf}
    \caption{Number of training tokens (on log scale) available from various chemical sources compared with typical LLM training runs. The numbers are drawn from ZINC\cite{irwin2012zinc}, PubChem\cite{kim2016pubchem}, \citet{touvron2023llama}, ChEMBL\cite{Gaulton2012-og}, and \citet{Kinney2023-fj}}.
    \label{fig:tokens}
\end{figure}

Regarding datasets, there are two types of data used for training LLMs: training data (unlabeled) and evaluation data (labeled). Training data should be grounded on real molecules to build the correct "prior belief" of a molecule definition during the LLM training process. Similar care is taken when natural language training data used in GPT-4, for instance, is built from real sentences or code, not random combinations of words that might be grammatically correct. 
Figure \ref{fig:tokens} shows the number of tokens on common chemistry datasets in comparison with the LLaMA 2 training data, extracted from \cite{irwin2012zinc, kim2016pubchem, touvron2023llama, Gaulton2012-og, Kinney2023-fj}. According to this data, the largest chemical training corpus, composed of hypothetical chemical structures, composes billions of tokens against a few trillion in the LLaMA 2 training data. 
Interestingly, \citet{segler2018planning} demonstrated that even using the Reaxys dataset, a very small human-curated set of chemical reactions, is enough to enable state-of-the-art retrosynthesis results. Therefore, the lack of data is not the only problem. Instead, the lack of good-quality data seems to be the pivotal factor holding back the development of better scientific LLMs. 
Figure \ref{fig:tokens} illustrates the number of tokens on ZINC, a dataset with hypothetical chemical structures\cite{irwin2012zinc}

On the other hand, benchmark data evaluates the success of these models. Numerous datasets, curated by the scientific community, are available for this purpose\cite{_jablonka_awesome-chemistry-datasets, Mirza2024-qw}. Among them, MoleculeNet\cite{wu_moleculenet_2018}, first published in 2017, is the most commonly used labeled dataset for chemistry. However, MoleculeNet has several issues: it is small, contains errors and inconsistencies, and lacks relevance to real-world chemistry problems\cite{Gloriam2019-yf, irwin_chemformer_2022, liu_multi-modal_2023, Livne2023-bu}. Pat Walters, a leader in ML for drug discovery, stated, “I think the best way to make progress on applications of machine learning to drug discovery is to fund a large public effort that will generate high-quality data and make this data available to the community”\cite{pat_walters_blog3}.

Walters also emphasized the need for relevant benchmarks. He noted that accurately predicting free energy solvation using the FreeSolv\cite{Mobley2014-mb} dataset does not lead to chemical discoveries. Relevant, truth-grounded datasets include the Absorption, Distribution, Metabolism, and Excretion (ADME) data curated by \citet{Fang2023-aj} and the Therapeutic Data Commons (TCD)\cite{TDC-ss, Huang2021-ug}. These datasets contain measurements of real compounds, making them grounded in reality. Moreover, ADME is crucial for determining a drug candidate’s success, while therapeutic results in diverse modalities align with metrics used in drug development.

Here, we hypothesize that the lack of easily accessible, high-quality data in the correct format for training foundational chemical language models is a major bottleneck to the development of the highly desired ``super-human'' AI-powered digital chemist. In addition, we argue that extracting data from scientific chemistry papers might be an interesting commitment to generating data of high quality, grounded to the truth, and on a large scale.


% \input{LLM_fig}
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figs/llm_applications.png}
    \caption{Classification of LLMs in chemistry and biochemistry according to their application. }
    \label{fig:applications}
\end{figure}


\begin{figure}
    \centering
    % \includesvg[width=\textwidth]{figs/llm_ldt.svg}
    \includegraphics[height=\textwidth, angle=90]{figs/llm_ldt.png}
    \caption{Illustration of how Large Language Models (LLMs) evolved chronologically.}
    \label{fig:sci_llms}
\end{figure}


\subsection{Property Prediction and Encoder-only mol-LLMs}\label{sec:sciEncoder}

\begin{table*}[ht]
    \small
    \caption{\ Encoder-only scientific LLMs.
    $a$:``Model Size'' is reported as the number of parameters.
    $b$: The authors report they not used as many encoder layers as it was used in the original BERT paper. But the total number of parameters was not reported.}
    \label{tab:enc_llms}
    \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}m{2.8cm}|m{1.5cm}m{4cm}m{1.5cm}m{3.5cm}m{2cm}}
        LLM   & Model Size$^a$ & Training Data & Architecture & Application & Release date\\\hline
        CatBERTa\cite{ock_catalyst_2023}
        & 355M & OpenCatalyst2020 (OC20) & RoBERTa & Property prediction & 2023.11 \\
        MaterialsBERT\cite{Yoshitake2022-xh} 
        & 110M & 2.4M material science abstracts + 750 annotated abstract for NER & BERT & NER and property extraction & 2023.04 \\
        SolvBERT\cite{Yu2022-fr}
        & \textit{b} & 1M SMILES of solute-solvent pairs from CombiSolv-QM & BERT & Property prediction & 2023.01 \\
        ChemBERTa-2\cite{ahmad_chemberta-2_2022}
        & 5M - 46M & 77M SMILES from PubChem & RoBERTa & Property prediction & 2022.09\\
        ScholarBERT\cite{Hong2022-mv} 
        &340M, 770M& Public.Resource.Org, Inc &BERT& Property prediction & 2022.05 \\
        MatSciBERT\cite{Gupta2022-hy} 
        & 110M & $\sim$150K material science paper downloaded from Elsevier & BERT & NER and text classification & 2022.05 \\
        MatBERT\cite{Trewartha2022-ez} 
        & 110M & Abstracts from solid state articles and abstracts and methods from gold nanoparticle articles & BERT & NER & 2022.04 \\
        PubMedBERT\cite{Gu2021-yn} 
        & 110M & 14M abstracts from PubMed & BERT & NER, QA, and document classification & 2021.10 \\
        Mol-BERT\cite{Li2021-xw}
        & 110M & $\sim$4B SMILES from ZINC15 and ChEMBL27 & BERT & Property prediction & 2021.09 \\
        ChemBERT\cite{Guo2022-kr}
        & 110M & $\sim$200k extracted using ChemDataExtractor & BERT & NER & 2021.06 \\
        MolBERT\cite{Fabian2020-zd} 
        & $\sim$85M & ChemBench & BERT & Property prediction & 2020.11\\
        ChemBERTa\cite{Chithrananda2020-cd}
        &  & 10M SMILES from PubChem & RoBERTa & Property prediction & 2020.10\\
        BioMegatron\cite{Shin2020-cp}
        & 345M, 800M, 1.2B &Wikipedia, CC-Stories,  Real-News,  and  OpenWebtext& Megatron-LM & NER and QA & 2020-10 \\
        BioBERT\cite{Lee2020-vl} 
        & 110M & PubMed and PMC & BERT & NER and QA & 2020.02 \\
        SciBERT\cite{Beltagy2019-ri} 
        & 110M &  1.14M papers from Semantic Scholar & BERT & NER and sentence classification & 2019.09 \\
        SMILES-BERT\cite{Wang2019-nq}
        & $b$ & 18,671,355 SMILES from ZINC & BERT & Property prediction & 2019.09\\
        BlueBERT\cite{Peng2019-yb} 
        & 110M & PubMed and MIMIC-III & BERT & NER, and document classification & 2019.06 \\
        ClinicalBERT\cite{Huang2019-gw} 
        & 110M & MIMIC-III & BERT & Pacient readmission probability & 2019.04 \\
    \end{tabular*}
\end{table*}


Encoder-only transformer architectures solely comprise an encoder. Chemists can leverage the simpler encoder-only architecture for tasks where the primary goal is classification, efficient exploration of chemical space, and property prediction. Since encoder-only architectures are mostly applied to property prediction, we describe here the relative importance of this principal chemical challenge.

\subsubsection{Property Prediction}

The universal value of chemistry lies in identifying and understanding properties of compounds to optimize their practical applications. In the pharmaceutical industry, therapeutic molecules interact with the body in profound ways.\cite{wu_bloodbrain_2023, bissantz2010medicinal, roughley2011medicinal} Understanding these interactions and modifying molecular structures to enhance those therapeutic benefits can lead to significant medical advancements.\cite{doytchinova_drug_2022} Similarly, in polymer science, material properties depend on chemical structure, polymer chain length, and packing,\cite{intro_to_polymer_science} and a protein’s function similarly depends on its structure and folding.
Historically, chemists have identified new molecules from natural products\cite{newman_natural_2016} and screened them against potential targets\cite{ferreira_drug_2023} to test their properties for diseases. Once a natural product shows potential, chemists synthesize scaled-up quantities for further testing or derivatization,\cite{kolb_growing_2003, castellino_late-stage_2023, sharma_peptide-based_2023} a costly and labor-intensive process.\cite{reizman_feedback_2016, dimasi_innovation_2016}
Traditionally, chemists have used their expertise to hypothesize the properties of new molecules derived from those natural products, hence aiming for the best investment of synthesis time and labor.
To support the chemical industry in more accurate property prediction, computational chemistry has evolved.\cite{lewars_computational} Quantum theoretical calculations predict certain properties reliably, while force-field-based Molecular Dynamics (MD)\cite{brini_adapting_2016} predict packing and crystal structures of large molecular ensembles, though both require substantial computational resources.\cite{bidault_how_2023, pyzer-knapp_accelerating_2021,fredericks_pyxtal_2021, case_convergence_2016, kazantsev_efficient_2011}
Property prediction can now be enhanced through machine learning tools,\cite{huang_application_2023, shilpa_recent_2023, martinez-mayorga_pursuit_2024, Wellawatte2023-uv} and more recent advancements in large language models lead to effective property prediction without the extensive computational demands of quantum mechanics and MD calculations. Combined with human insight, AI can revolutionize material development, enabling the synthesis of new materials with a high likelihood of possessing desired properties for specific applications.


%\begin{figure}[h!]
%    \centering
%    \includegraphics[width=0.6\textwidth]{figs/transformers_in_chemistry_combined_v2.png}
%    \caption{a) encoder-decoder transformers have been traditionally used for translation tasks, and for chemistry are predominantly used in reaction prediction, where a set of reactants is translated into a set of products. b) encoder-only transformers provide a vector output and have been traditionally used for sentiment analysis. In chemistry, they are predominantly used in property prediction or classification tasks. c) decoder-only transformers generate an inference, or a set of likely next tokens in a sequence. In chemistry, they are predominantly used to extrapolate to modified or larger molecules beyond a set of input molecules.}
%    \label{fig:transformers_in_chem}
%\end{figure}

\subsubsection{Encoder-only Mol-LLMs}

Encoder-only models are exemplified by the BERT architecture, which is commonly applied in natural language sentiment analysis to extract deeper patterns from prose.\cite{deng_llms_2023} The human chemist has been taught to look at a 2D image of a molecular structure and to recognize its chemical properties or classify the compound. Therefore, encoder-only models would ideally convert SMILES strings, empty of inherent chemical essence, into a vector representation, or latent space, reflecting those chemical properties. This vector representation can then be used directly for various downstream tasks.

\citet{Schwaller2020-xh} used a BERT model to more accurately classify complex synthesis reactions by generating reaction fingerprints from raw SMILES strings, without the need to separate reactants from reagents in the input data, thereby simplifying data preparation. The BERT model achieved higher accuracy (98.2\%) compared to the encoder-decoder model (95.2\%) for classifying reactions. Accurate classification aids in understanding reaction mechanisms, vital for reaction design, optimization, and retrosynthesis. \citet{Toniato2023-in} also used a BERT architecture to classify reaction types for downstream retrosynthesis tasks that enable manufacture of any molecular target. Further examples of BERT use include unsupervised reaction atom-to-atom mapping \cite{schwaller_extraction_2021, Schwaller2021-vo}. These chemical classifications would accelerate research and development in organic synthesis, described further below.

Due to limited labeled data for molecular property prediction, \citeauthor{wang_smiles-bert_2019} proposed a semi-supervised SMILES-BERT model, pre-trained on a large unlabeled dataset with a Masked SMILES Recovery task.\cite{wang_smiles-bert_2019} The model was then fine-tuned for various molecular property prediction tasks, outperforming state-of-the-art methods in 2019 on three chosen datasets varying in size and property. This marked a shift from using BERT for reaction classification towards property prediction and drug discovery.

\citet{Zhang2022-ar} also tackled the issue of limited property-labeled data and the lack of correlation between any two datasets labeled for different properties, hindering generalizability. They introduced multitask learning BERT (MTL-BERT), which used large-scale pretraining and multitask learning with unlabeled SMILES strings from ChEMBL.\cite{Gaulton2012-og} This approach mined contextual information and extracted key patterns from complex SMILES strings, improving model interpretability. The model was fine-tuned for relevant downstream tasks, achieving better performance than state-of-the-art methods in 2022 on 60 molecular datasets from ADMETlab\cite{Xiong2021-lf} and MoleculeNet.\cite{wu_moleculenet_2018}

In 2021, \citeauthor{Li2021-xw}\cite{Li2021-xw} introduced Mol-BERT, pre-trained on four million unlabeled drug SMILES from the ZINC 15\cite{sterling_zinc_2015} and ChEMBL 27\cite{Gaulton2012-og} databases to capture molecular substructure information for property prediction. Their work leveraged the underutilized potential of large unlabeled datasets like ZINC. Mol-BERT consisted of three components: PretrainingExtractor, Pretraining Mol-BERT, and Fine-Tuning Mol-BERT. It treated Morgan fingerprint fragments as "words" and compounds as "sentences," using RDKit and the Morgan algorithm for canonicalization and substructure identification. This approach generated comprehensive molecular fingerprints from SMILES strings, used in a Masked Language Model (MLM) task for pretraining. Mol-BERT was fine-tuned on labeled samples, providing outputs as binary values or continuous scores for classification or regression, and it outperformed existing sequence and graph-based methods by at least 2\% in ROC-AUC scores on Tox21, SIDER, and ClinTox datasets.\cite{wu_moleculenet_2018}

\citet{Ross2022-xf} introduced MoLFormer, a large-scale unsupervised BERT model for more accurate and faster molecular property predictions than Density Functional Theory calculations or wet-lab experiments. They trained MoLFormer with rotary positional embeddings on SMILES sequences of 1.1 billion unlabeled molecules from PubChem\cite{kim2016pubchem} and ZINC\cite{sterling_zinc_2015}. Rotary positional encoding captures token positions more effectively than traditional methods, \cite{Vaswani2017-kq} improving modeling of sequence relationships. MoLFormer outperformed state-of-the-art Graphical Neural Networks on several classification and regression tasks from ten MoleculeNet\cite{wu_moleculenet_2018} datasets, while performing competitively on two others. It effectively learned spatial relationships between atoms, predicting various molecular properties, including quantum-chemical properties. Additionally, MoLFormer significantly increased efficiency, reducing GPU usage by a factor of 60 (16 GPUs instead of 1000).

With ChemBERTa, \citet{Chithrananda2020-cd} explored the impact of pretraining dataset size, tokenization strategy, and the use of SMILES or SELFIES, distinguishing their work from other BERT studies. They used HuggingFace's RoBERTa transformer,\cite{wolf2020huggingfaces}  and referenced a DeepChem\cite{wu_moleculenet_2018} tutorial for accessibility. Their results showed improved performance on downstream tasks (BBBP, ClinTox, HIV, Tox21 from MoleculeNet\cite{wu_moleculenet_2018}) as the pretraining dataset size increased from 100K to 10M. Although ChemBERTa did not surpass state-of-the-art GNN-based baselines like Chemprop (which used 2048-bit Morgan Fingerprints from rdkit),\cite{yang_analyzing_2019} the authors suggested that with expansion to larger datasets they would eventually beat those baselines. The authors compared Byte-Pair Encoder (BPE) with a custom SmilesTokenizer and its regex developed by Schwaller et al.\cite{Schwaller2019-lc} while exploring tokenization strategies. They found the SmilesTokenizer slightly outperformed BPE, suggesting more relevant sub-word tokenization is beneficial. No difference was found between SMILES and SELFIES, but the paper highlighted how attention heads in transformers could be visualized with BertViz,\cite{vig2019bertviz} showing certain neurons selective for functional groups. This study underscored the importance of appropriate benchmarking and addresses the carbon footprint of AI in molecular property prediction.


In ChemBERTa-2, \citet{ahmad_chemberta-2_2022} aimed to create a foundational model applicable across various tasks. They addressed criticisms of biased data in large language models by training on 77M samples and adding a Multi-Task Regression component to the pretraining. ChemBERTa-2 matched state-of-the-art architectures on MoleculeNet.\cite{wu_moleculenet_2018} As with ChemBERTa, the work was valuable because of additional exploration, in this case into how pretraining improvements affected certain downstream tasks more than others, depending on the type of fine-tuning task, the structural features of the molecules in the fine-tuning task data set, or the size of that fine-tuning dataset. The result was that pretraining the encoder-only model is important, but gains could be made by considering the chemical application itself, and the associated fine-tuning dataset.

The paper acknowledged additional graph-based transformer pretraining approaches, like Node Attribute Masking, and suggested hybrid molecular representations. It also foreshadowed contrastive learning, as proposed by \citet{guan_t-mgcl_2023}. Contrastive learning is a self-supervised approach where a model learns useful data representations by contrasting similar and dissimilar sample pairs, generated through data augmentation. Data augmentation increases data diversity by adding modified copies of the original data.\cite{schwaller2020data, ding_data_2024} Since graph structures vary greatly depending on the research field and whether small molecule or proteins are being studied, for example, there is no single universal augmentation method. Therefore augmentation strategies include atom masking, bond deletion, subgraph removal, and attribute masking. 

In June 2023, \citet{Yuksel2023-iy} introduced SELFormer, building on ideas from ChemBERTa2\cite{ahmad_chemberta-2_2022} and using SELFIES for large data input. Yüksel et al. argue that SMILES strings have validity and robustness issues, hindering effective chemical interpretation of the data. SELFormer uses SELFIES and is pre-trained on two million drug-like compounds, fine-tuned for diverse molecular property prediction tasks (BBBP, SIDER, Tox21, HIV, BACE, FreeSolv, ESOL, PDBbind from MoleculeNet).\cite{wu_moleculenet_2018} SELFormer outperformed all competing methods for some tasks and produced comparable results for the rest. It could also discriminate molecules with different structural properties. The paper suggests future directions in multimodal models combining structural data with other types of molecular information including text-based annotations. We will discuss such multimodal models below.

Also in 2023, \citet{Yu2022-fr} published SolvBERT, a multi-task BERT-based regression model that could predict both solvation free energy and solubility from the SMILES notations of solute-solvent complexes. It was trained on the CombiSolv-QM dataset,\cite{vermeire2021transfer} a curation of experimental solvent free energy data called CombiSolv-Exp-8780,\cite{Mobley2014-mb, marenich2020minnesota, moine2017estimation, grubbs2010mathematical} and the solubility dataset from \citet{boobier2020machine}. SolvBERT's performance was benchmarked against advanced graph-based models like the Directed Message Passing Neural Network (D-MPNN)\cite{yang2019learned} and a newer GNN–Transformer hybrid model, GROVER.\cite{Rong2020-as} This work is powerful because there is an expectation that solvation free energy depends on 3-dimensional conformational properties of the molecules, or at least 2D properties that would be well characterized by graph-based molecular representations. SolvBERT showed comparable performance to DMPNN in predicting solvation free energy, largely due to its effective clustering feature in the pre-training phase as shown by TMAP visualizations. Furthermore, SolvBERT outperformed GROVER in predicting experimentally evaluated solubility data for new solute–solvent combinations. This underscores the significance of how SolvBERT seemed capable of capturing the dynamic and spatial complexities of solvation interactions in a text-based model.

While significant progress has been made, in 2024, Jiang et al. still discuss the limitations of labeled data and introduce INTransformer,\cite{jiang_intransformer_2024} a transformer-based molecule property prediction method. It enhances the ability to capture global information from molecules by adding perturbing noise and using contrastive learning, artificially augmenting smaller datasets. This approach achieved higher performance, and work with smaller datasets using various transformer strategies is ongoing.


\subsection{Property Directed Inverse Design and Decoder-only mol-LLMs}\label{sec:SciDecoder}

\begin{table*}[ht]
    \small
    \caption{\ Decoder-only scientific LLMs. $a$:``Model Size'' is reported as the number of parameters. ``PubMed'' refer to the PubMed abstracts dataset, while PMC (PubMed Corpus) refers to the full-text corpus dataset.}
    \label{tab:dec_llms}
    \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}m{2.5cm}|m{1.5cm}m{4cm}m{1.5cm}m{3.5cm}m{2cm}}
        LLM   & Model Size$^a$ & Training Data & Architecture & Application & Release date\\\hline
        % 3M-Diffusion\cite{zhu_3m-diffusion_2024}
        % && 300K molecule-text pairs from PubChem &&& 2024.03 \\
        BioMedLM\cite{Bolton2024-al}
        & 2.7B & PubMed abstracts and full articles & GPT & QA & 2024.03\\
        BioMistral\cite{Labrak2024-xs} 
        & 7B & PubMed Central (PMC) & Mistral & QA & 2024.02 \\
        BiMediX\cite{Pieri2024-jy}
        & 8x7B & 1.3M Arabic-English instructions (BiMed) & Mixtral & QA & 2024.02\\
        EpilepsyLLM\cite{Zhao2024-hi} 
        & 7B & Data from the Japan Epilepsy Association, Epilepsy Information Center, and Tenkan Net & LLaMa & QA & 2024.01 \\
        ChemSpaceAL\cite{kyro_chemspaceal_2024}
        &  & ChEMBL 33, GuacaMol v1, MOSES, and BindingDB 08-2023 & GPT & Molecule Generation & 2024.01 \\
        CheXagent\cite{Chen2024-lg}
        & 7B & 28 publicly available datasets, including PMC, MIMIC, wikipedia, PadChest, and BIMCV-COVID-19 & Mistral & QA, Image understanding & 2024.01 \\
        BioMedGPT-LM\cite{Luo2023-gw} 
        & 7B and 10B & 5.5M biomedical papers from S2ORC & LLaMA2 & QA & 2023.08 \\
        Darwin\cite{Xie2023-nh} 
        & 7B & SciQ and Web of Science & LLaMA & QA, Property prediction, NER, and Molecule Generation & 2023.08 \\ %also 16 physical-chemistry props dataset
        cMolGPT\cite{Wang2023-jd}
        &  & MOSES & GPT & Molecule Generation & 2023.04 \\
        PMC-LLaMA\cite{Wu2023-tb} 
        & 7B and 13B & MedC-k and MedC-I & LLaMA & QA & 2023.04 \\
        % CLAMP\cite{seidl_enhancing_2023}
        % &&&&& 2023.03 \\
        % BioTranslator\cite{xu_multilingual_2023}
        % &  &  & PubMedGPT & Molecule Generation & 2023.02 \\
        Galactica\cite{Taylor2022-pu} 
        &125M, 1.3B, 6.7B, 30B, 120B&The galactica corpus, a curation with ~62B scientific documents& Decoder-only & QA, NER, Document Summarization, Property Prediction & 2022.11 \\
        BioGPT\cite{Luo2022-sv} 
        & 355M & 15M of Title and abstract from PubMed & GPT-2 & QA, NER, and Document Classification & 2022-09 \\
        Adilov2021\cite{Adilov2021-ih}
        & 13.4M & 5M SMILES from ChemBERTa’s PubChem-10M. & GPT-2 & Property prediction and molecule generation & 2021.09 \\
        % AI-cell\cite{chandler_artificial_2022}
        % &&&&& \\
        % AutoMolDesigner\cite{shen_automoldesigner_2024}
        % &&&&& \\
        % DrugAssist\cite{}
        % &&&&& \\
        % CONSMI\cite{qian_consmi_2024}
        % &&&&& \\
        % CRTMorgan\cite{wang_explore_2023}
        % &&&&& \\
        % DockingGA\cite{gao_dockingga_2024}
        % &&&&& \\
        % Galactica\cite{Taylor2022-pu}
        % &&&&& \\
        % GIT-Mol\cite{Liu_2024_gitmol}
        % &&&&& \\
        % GPTChem\cite{Jablonka2023-bm}
        % &&&&& \\
        % Haroon2023\cite{haroon_generative_2023}
        % &&&&& \\
        % INTransformer\cite{jiang_intransformer_2024}
        % &&&&& \\
        % iupacGPT\cite{Mao2023-bo}
        % &&&&& \\
        % LLaVa-Med\cite{}
        % &&&&& \\
        % MediSwift\cite{Thangarasa2024-wb}
        % &&&&& \\
        % MolFormer\cite{Ross2022-yp} 
        % &&&&& \\
        % Molecular Transformer\cite{Schwaller2019-lc} 
        % &&&&& \\
        % MOLGEN\cite{Fang2023-ty}
        % &&&&& \\
        % MolGPT\cite{Bagal2022-tg}
        % &&&&& \\
        % MolTC\cite{fang_moltc_2024}
        % &&&&& \\
        % MolXPT\cite{liu_molxpt_2023}
        % &&&&& \\
        % MTL-BERT\cite{jia_all--one_2021}
        % &&&&& \\
        % MULTIMODAL-MOLFORMER\cite{soares_beyond_2023}
        % &&&&& \\
        % PeTrans\cite{wang_petrans_2023}
        % &&&&& \\
        % PremuNet\cite{zhang_pre-trained_2024}
        % &&&&& \\
        % Regression Transformer\cite{Born2023-nc}
        % &&&&& \\
        % Schwaller2020\cite{Schwaller2020-xh}
        % &&&&& \\
        % Schwaller2021\cite{schwaller_extraction_2021}
        % &&&&& \\
        % Schwaller2023\cite{Schwaller2021-vo}
        % &&&&& \\
        % SELFormer\cite{Yuksel2023-iy}
        % &&&&& \\
        % SGPT-RL\cite{xu_optimization_2024}
        % &&&&& \\
        % SolTranNet\cite{Francoeur2021-pu}
        % &&&&& \\
        % SolvBERT\cite{Yu2022-fr}
        % &&&&& \\
        % T-MGCL\cite{guan_t-mgcl_2023}
        % &&&&& \\
        % Taiga\cite{Mazuz2023-gb}
        % &&&&& \\
        % Text2Mol\cite{edwards-etal-2021-text2mol}
        % &&&&& \\
        % TGM-DLM\cite{gong_text-guided_2024}
        % &&&&& \\
        % Thomas2022\cite{thomas_augmented_2022}
        % &&&&& \\
        % Toniato2023\cite{Toniato2023-in}
        % &&&&& \\
        % TransAntivirus\cite{mao_transformer-based_2024}
        % &&&&& \\
        % Transformer-VAE\cite{yoshikai_novel_2024}
        % &&&&& \\
        % TransPolymer\cite{xu_transpolymer_2023}
        % &&&&& \\
        % TSMMG\cite{zhou_instruction_2024}
        % &&&&& \\
    \end{tabular*}
\end{table*}
%\textcolor{blue}{need to cite \cite{Jablonka2023-bm}}\todo{That was the chemRxiv paper. I updated it for the version published in Nature. Just make sure all the text refers to the updated text} THIS IS NOW DONE, BUT SINCE THE JABLONKA PAPER IS A NATURAL LANGUGAE DECODER-ONLY LLM, I USE THIS PAPER AS A SEGUE TO BRIDGE THE SECTIONS STILL TO COME. SEE AT THE END OF THIS SECTION. 
Decoder-only GPT-like architectures offer significant value for property directed molecule generation and \textit{de novo} chemistry applications because they excel in generating novel molecular structures by learning from vast datasets of chemical compounds, and capture intricate patterns and relationships within molecular sequences. They thus propose viable new compounds that adhere to desired chemical properties and constraints, enabling rapid exploration and innovation within an almost infinite chemical space. We first describe property directed inverse design from a chemistry perspective, and then go on to provide examples of how decoder-only LLMs have propelled inverse design forward. 

\subsubsection{Property Directed Inverse Design}

Nature has been a significant source of molecules that inhibit disease proliferation, as organisms have evolved chemicals to protect themselves. This has led to most pharmaceuticals being derived from natural products,\cite{li_drug_2009, newman_natural_2012} which offer advantages such as cell permeability, target specificity, and a vast chemical diversity.\cite{afarha_strategies_2016}
However, despite these benefits, there are high costs and complexities associated with high-throughput screening and synthesis of natural products.\cite{afarha_strategies_2016, li_drug_2009}
%Despite the benefits of natural products, the pharmaceutical industry reduced its focus on them due to the high costs and complexities associated with high-throughput screening and synthesis, but thereafter, a shift towards synthetic compounds coincided with a decrease in new drug approvals.\cite{afarha_strategies_2016} Emerging methods in tracking biodiversity and advancements in synthetic biology have since revived interest in natural product-based drug discovery.\cite{li_drug_2009}
While building on the chemical diversity and efficacy of natural products, AI also opens new avenues for synthesizing unique compounds efficiently. Advanced \textit{in-silico} molecular design allows for rapid mutation\cite{nigam_beyond_2021} towards valid \textit{de-novo} molecular structures that are synthesizable,\cite{Wellawatte2023-uv, Gandhi2022-mx} streamlining the iterative process of drug development. Yet, the true innovation lies in the potential of LLM-driven target-directed molecular design or "Inverse Design," where we can start with a desired property and directly generate molecules that manifest this attribute, bypassing traditional stepwise modifications. This capability dramatically accelerates the pathway from concept to viable therapeutic agents and aligns well with decoder-only LLM architectures.

%Nature has significantly contributed to generating molecules that restrict disease proliferation in that the organisms have evolved chemicals to protect themselves. Hence, most pharmaceuticals have been derived from natural products.\cite{li_drug_2009, newman_natural_2012}
%Working with natural products offers benefits such as cell permeability, target specificity, and vast chemical diversity.\cite{afarha_strategies_2016}. However, \citet{afarha_strategies_2016} report how the pharmaceutical industry reduced its focus on natural products due to costly complexities in high-throughput screening and synthesis. The industry shifted to synthetic compounds, but this correlated with fewer new drug approvals. Improved methods for tracking biodiversity and synthetic biology are now reviving interest in natural product-based drug discovery.\cite{li_drug_2009}

%Regardless of advancements in screening natural products and synthetic chemical libraries, there remains a reliance on natural products that can actually be addressed through \textit{in-silico} and \textit{de-novo} molecular design. Molecular mutation can be achieved by modifying chemical representations,\cite{nigam_beyond_2021} ensuring new molecules are valid and synthesizable.\cite{Wellawatte2023-uv, Gandhi2022-mx} The goal is to design previously unknown molecules against specific targets, known as target-directed molecular design or "Inverse Design." One approach is to generate or to mutate existing ones and then predict their properties. This is time-consuming as properties must subsequently be predicted for each generated molecule. Ideally, therefore, inverse design would go directly from target properties to molecules likely to meet those properties, presenting a significant challenge for AI and LLMs in chemistry, aligning well with decoder-only LLM architectures.

\subsubsection{Decoder-only mol-LLMs}

In 2021, \citet{Adilov2021-ih} presented "Generative pretraining from Molecules," one of the first applications of decoder-only models to SMILES strings. It pre-trained a GPT-2-like causal transformer for self-supervised learning, introducing "adapters" between attention blocks for task-specific fine-tuning.\cite{houlsby2019parameter} This method, requiring minimal architectural changes, offered versatility in molecule generation and property prediction, aiming to surpass ChemBERTa's encoder-only performance with a more scalable and resource-efficient approach. Another early decoder-only SMILES-based model was Bagal et al's MolGPT model,\cite{Bagal2022-tg}. MolGPT, with a mere 6 million parameters, advanced GPT-type LLMs for molecular generation. Its decoder-only architecture with masked self-attention facilitated learning long-range dependencies, enabling chemically valid SMILES representations that met complex structural rules involving valency and ring closures. The paper also used salience measures for interpretability in predicting SMILES tokens. MolGPT outperformed many existing Variational Auto-Encoder (VAE) based approaches\cite{fuhr_deep_22, han_revolutionizing_23, koutroumpa_systematic_23, kell_deep_20, bilodeau_generative_22, gangwal_generative_24, vogt_using_22, talluri_novel_24} in predicting novel molecules with specified properties, being trained on datasets like MOSES\cite{Polykovskiy2020-fv} and GuacaMol.\cite{Brown2019-ul} It showed good performance with metrics like validity, uniqueness, Frechet ChemNet Distance (FCD),\cite{preuer2018frechet} and KL divergence,\cite{Brown2019-ul} further details of which are described in the paper, allowing direct comparisons in the field. While MolGPT's computational demands might be higher than traditional VAEs, its ability to generate high-quality, novel molecules justifies this trade-off, but future research could likely optimize model efficiency or explore lighter versions. A brief summary of advancements in transformer-based models for \textit{de-novo} molecule generation from 2023, and 2024 follow.


\citet{haroon_generative_2023} further developed a GPT-based model with relative attention for \textit{de novo} drug design, showing improved validity, uniqueness, and novelty. Both \citet{wang_explore_2023} and \citet{mao_transformer-based_2024} presented work that surpassed MolGPT, with Mao et al.'s T5-type model\cite{raffel_exploring_2020}  generating novel compounds using IUPAC names directly.\cite{Mao2023-bo} Although T5-based, we include this here because of its relevance to \textit{de novo} drug design.
In a similar vein, \citet{zhang_simple_2023} proposed including target 3D structural information in molecular generative models, even though their approach is not LLM-based. However, we nonetheless note its value for future structure-based LLM drug design. They demonstrated that integrating additional biological data significantly enhances the relevance and specificity of generated molecules for targeted drug discovery.
\citet{wang_petrans_2023} discussed PETrans, a deep learning method for generating target-specific ligands using protein-specific encoding and transfer learning. This study emphasized the application of transformer models for generating molecules with a high binding affinity to specific protein targets. 

In 2024, \citet{yoshikai_novel_2024} discussed the limitations of transformer architectures in recognizing chirality from SMILES representations, highlighting the challenges in learning overall molecular structures with, in particular, chirality impacting the prediction accuracy of molecular properties. They coupled a transformer with a VAE to address this. \citet{qian_consmi_2024} introduced CONSMI, motivated by contrastive learning in NLP, to generate new molecules using multiple SMILES representations, improving molecular novelty and validity. \citet{kyro_chemspaceal_2024} presented ChemSpaceAL, an active learning method for protein-specific molecular generation, efficiently discovering molecules with desired characteristics without prior knowledge of existing inhibitors. \citet{yan_predicting_2024} proposed the GMIA framework, featuring a graph mutual interaction attention decoder for drug-drug interaction prediction, enhancing prediction accuracy and interpretability. Lastly, \citet{shen_automoldesigner_2024} reported on AutoMolDesigner, an AI-based open-source software for automated design of small-molecule antibiotics, emphasizing a user-friendly interface and potential for accelerating antibiotic discovery.

For a deeper dive into decoder-only transformer architecture in chemistry, we highlight the May 2023 "Taiga" model by \citet{Mazuz2023-gb}, and cMolGPT by \citet{Wang2023-jd}. Taiga first learns to map SMILES strings to a vector space, and then refines that space using a smaller dataset of labeled molecules to produce molecules with targeted attributes. It employs an autoregressive mechanism, sequentially predicting each SMILES character based on the previous ones. For optimizing molecular properties, Taiga uses the REINFORCE algorithm\cite{Zhang2020-ji}, which develops a strategy to enhance desired molecular features. Although this fine-tuning with reinforcement learning (RL) slightly reduces molecule validity, it significantly boosts their practical applicability. Initially evaluated using the Quantitative Estimate of Drug-likeness (QED) metric,\cite{bickerton2012quantifying} Taiga has also demonstrated promising results in targeting IC50 values,\cite{Gaulton2012-og} the BACE protein,\cite{subramanian2016computational} and anti-cancer activities they collected from a variety of sources. This work underscores the importance of using new models to address applications that require a higher level of chemical sophistication, to illustrate how such models could ultimately be applied outside of the available benchmark datasets. It also builds on the necessary use of standardized datasets and train-validation-test splitting, to demonstrate progress, as explained by \citet{wu_moleculenet_2018}. Yet, even the MoleculeNet benchmarks\cite{wu_moleculenet_2018} are flawed and we point the reader here to a more detailed discussion on benchmarking,\cite{pat_walters_blog3} given that a significant portion of molecules in the BACE dataset have undefined stereo centers, which, at a deeper level, complicates the modeling and prediction accuracy.

\citet{Wang2023-jd} introduced "cMolGPT: A Conditional Generative Pre-Trained Transformer for Target-Specific \textit{de novo} Molecular generation," which underscores the importance of incorporating chemical domain knowledge to effectively navigate the vast landscape of drug-like molecules. Using unsupervised learning and an auto-regressive approach, cMolGPT generates SMILES guided by predefined conditions based on target proteins and binding molecules. Initially trained on the MOSES dataset\cite{Polykovskiy2020-fv} without target information, the model is fine-tuned with embeddings of protein-binder pairs, focusing on generating compound libraries and target-specific molecules for the EGFR, HTR1A, and S1PR1 protein datasets.\cite{xu20084, yu2022structural, xu2021structural, sun2017excape}

Their approach employs a QSAR model\cite{yang_concepts_2019} to predict the activity of generated compounds, achieving a Pearson correlation coefficient over 0.75. However, reliance on this QSAR model, which has its own limitations, underscores the necessity for more extensive experimental datasets. Despite its capabilities, the cMolGPT model tends to generate molecules within the confines of the same sub-chemical space as the original dataset, indicating that while it successfully identifies potential binders, it faces challenges in broadly exploring the chemical space to discover novel solutions. This limitation highlights the difficulty of generating molecules from significantly different chemical families that are effective in binding or possess a combination of desired properties, suggesting a need for approaches that can more effectively expand the exploration of chemical diversity.
Regardless, models capable of this kind of conditional generation are typically trained on large datasets of known protein-ligand interactions. Through this training, they learn the complex relationship between protein structures and the chemical structures of binding ligands. The model learns to predict which molecular features or structures are important for interacting with proteins that have certain characteristics (as captured in the embeddings).
While both "Taiga" and "cMolGPT" use transformer architectures and decoder-only setups for molecule generation, they differ in approach. Taiga integrates reinforcement learning to optimize its generative model, while cMolGPT uses target-specific embeddings to guide the generation process.

Outside of training on SMILES strings, \citet{Mao2023-bo} introduce iupacGPT, which also uses a decoder-only architecture, modeled after GPT-2. It addresses the limitations of SMILES strings by using IUPAC names to integrate human-readable chemical semantics. It focuses on pretraining with a vast IUPAC dataset and fine-tuning with lightweight networks, excelling in molecule generation, classification, and regression tasks.

We also refer the reader to several other good reviews, \cite{guzman-pando_deep_2023, fromer_computer-aided_2023, vogt_exploring_2023-1, Das2024-ad} with \citet{goel_efficient_2023} exploring the efficiency of modern machine learning methods in sampling drug-like chemical space for virtual screening and molecular design. The work of \citet{goel_efficient_2023} discussed generative models, including LLM approaches, for approximating the entire drug-like chemical space and highlighted models conditioned on specific properties or receptor structures. 

We provide a segue from this section by introducing the work by \citet{Jablonka2023-bm}, which showcases a decoder-only GPT model that, despite its training on natural language rather than specialized chemical languages, competes effectively with decoder-only LLMs tailored to chemical languages. The authors use GPT-3 to answer complex chemistry questions and therefore highlight its potential as a foundational tool in the field. This sets the stage for integrating a natural language decoder-only LLM, like ChatGPT, into chemical research, where it could serve as a central hub. This foreshadows future developments to pair the LLM with specialized tools to enhance capabilities, paving the way for the creation of autonomous agents that leverage deep language understanding in scientific domains.

\subsection{Synthesis Prediction and Encoder-decoder Mol-LLMs}\label{sec:sciEncDec}

\begin{table*}[ht]
    \small
    \caption{\ Encoder-decoder scientific LLMs.
    $a$:``Model Size'' is reported as the number of parameters.}
    \label{tab:enc_dec_llms}
    \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}m{2.5cm}|m{1.5cm}m{4cm}m{1.5cm}m{3.5cm}m{2cm}}
        LLM   & Model Size$^a$ & Training Data & Architecture & Application & Release date\\\hline
        BioT5+\cite{Pei2024-ph} 
        & 252M &ZINC20, UniRef50, 33M PubMed articles, 339K mol-text pairs from PubChem, 569K FASTA-text pairs from Swiss-prot& T5 & Molecule Captioning, Molecule Generation, Property Prediction,  & 2024-02 \\
        BioT5\cite{Pei2023-bp} 
        & 252M &ZINC20, UniRef50, full-articles from BioRxiv and PubMed, mol-text-IUPAC information from PubChem & T5 & Molecule Captioning, Property Prediction & 2023-12 \\
        ReactionT5\cite{Sagawa2023-fa}
        & 220M & ZINC and ORD & T5 & Property prediction and Reaction prediction & 2023.11 \\
        Text+Chem T5\cite{Christofidellis2023-ea}
        & 60M, 220M & 11.5M or 33.5M samples curated from \citet{Vaucher2020-gz}, \cite{Toniato2023-in}, and CheBI-20& T5 & Molecule Captioning, Product Prediction, Retrosynthesis, Molecule Generation & 2023.01 \\
        MolT5\cite{Edwards2022-yu} 
        & 60M, 770M & C4 dataset & T5 & Molecule Captioning and Molecule Generation & 2022.11 \\
        T5Chem\cite{Lu2022-ms}
        & 220M & USPTO & T5 & Product Prediction, Retrosynthesis, Property Prediction & 2022.03 \\
        ChemFormer\cite{irwin_chemformer_2022}
        & 45M, 230M & 100M SMILES from ZINC-15 & BART & Product Prediction, Property Prediction, Molecular Generation & 2022.01 \\
    \end{tabular*}
\end{table*}

The encoder-decoder architecture is designed for tasks involving the translation of one sequence into another, making it ideal for predicting chemical reaction outcomes or generating synthesis pathways from given reactants. We begin with a background on optimal synthesis prediction and describe how earlier machine learning has approached this challenge. Following that, we explain how LLMs have enhanced chemical synthesis prediction and optimization.

\subsubsection{Synthesis Prediction}

Once a molecule has been identified through property-directed inverse design, the next challenge is to predict its optimal synthesis, including yield. \citet{shenvi-2024-natural} describe how the demanding and elegant syntheses of natural products has contributed greatly to organic chemistry. However, in the past 20 years, the focus has shifted away from complex natural product synthesis towards developing reactions applicable for a broader range of compounds, especially in reaction catalysis.\cite{shenvi-2024-natural} Yet, complex synthesis is becoming relevant again as it can be digitally encoded, mined by LLMs, and applied to new challenges. Unlike property prediction, reaction prediction is challenging due to the involvement of multiple molecules. Modifying one reactant requires adjusting all others, with different synthesis mechanisms or conditions likely involved. Higher-level challenges exist for catalytic reactions and complex natural product synthesis.
Synthesis can be approached in two ways. Forward synthesis involves building complex target molecules from simple, readily available substances, planning the steps progressively. Retrosynthesis, introduced by E.J. Corey in 1988,\cite{corey_robert_1988} is more common. It involves working backward from the target molecule, breaking it into smaller fragments whose re-connection is most effective. Chemists choose small, inexpensive, and readily available starting materials to achieve the greatest yield and cost-effectiveness. For example, the first total synthesis of discodermolide\cite{nerenberg_total_1993} involved 36 such steps, a 24-step longest linear sequence, and a 3.2\% yield. There are many possible combinations for the total synthesis of a target molecule, and the synthetic chemist must choose the most sensible approach based on their expertise and knowledge. However, this approach to total synthesis takes many years.
LLMs can now transform synthesis such that structure-activity relationship predictions can be coupled in lock-step with molecule selection based on easier synthetic routes. This third challenge of predicting the optimal synthesis can also lead to the creation of innovative, non-natural compounds, chosen because of such an easier predicted sytnthesis but for which the properties are still predicted to meet the needs of the application. Thus, these three challenges introduced above are interconnected.

\subsubsection{Encoder-decoder mol-LLMs}
Before we focus on transformer use, some description is provided on the evolution from RNN and Gated Recurrent Unit (GRU) approaches in concert with the move from template-based to semi-template-based to template-free models. \citet{nam_linking_2016} pioneered forward synthesis prediction using a GRU-based translation model, while \citet{liu_retrosynthetic_2017} reported retro-synthesis prediction with a Long Short-Term Memory (LSTM) based seq2seq model incorporating an attention mechanism, achieving 37.4\% accuracy on the USPTO-50K dataset.\cite{schneider-2016-fingerprint} The reported accuracies of these early models highlighted the challenges of synthesis prediction, particularly retrosynthesis. \citet{schneider-2016-fingerprint} further advanced retrosynthesis by assigning reaction roles to reagents and reactants based on the product.

Evolving from RNNs and GRUs, the field progressed with the introduction of template-based models. \citet{Segler2017-dq} identified that computational "rule-based systems" often failed because they ignored the molecular context, resulting in "reactivity conflicts." They prioritized suitable transformation rules describing how atoms and bonds change during reactions, applied in reverse for retrosynthesis. They trained a model on 3.5 million reactions, achieving 95\% top-10 accuracy in retrosynthesis and 97\% for reaction prediction on a validation set of nearly 1 million reactions from the Reaxys database (1771-2015). Though not transformer-based, their work paved the way for LLMs in synthesis applications. However, template-based models rely on explicit reaction templates from known reactions, which limits their ability to predict novel reactions and they require manual updates for learning new data.

Semi-template-based models offered a balance between rigid template-based methods and flexible template-free approaches. They used interpolation or extrapolation within template-defined spaces to predict a wider range of reactions and to adjust based on new data. In 2021, \citet{somnath_learning_2021} introduced a graph-based approach recognizing that precursor molecule topology is largely unchanged during reactions. Their model broke the product molecule into "synthons" and added relevant leaving groups, making results more interpretable.\cite{Wellawatte2023-rw} Training on the USPTO-50k dataset, \cite{schneider-2016-fingerprint} they achieved a top-1 accuracy of 53.7\%, outperforming previous methods.

It is, however, the template-free approaches that align well with transformer-based learning approaches because they learn retrosynthetic rules from raw training data. This provides significant flexibility and generalizability across various types of chemistry.  Template-free models are not constrained by template libraries and so can uncover novel synthetic routes that are undocumented or not obvious from existing reaction templates.
To pave the way for transformer use in synthesis, \citet{cadeddu_organic_2014} drew an analogy between fragments in a compound and words in a sentence due to their similar rank distributions. \citet{schwaller_found_2018} further advanced this with an LSTM network augmented by an attention-mechanism-based encoder-decoder architecture, using the USPTO dataset.\cite{schneider-2016-fingerprint} They introduced a commonly used "regular expression" (or "regex") for tokenizing molecules, framing synthesis (or retrosynthesis) predictions as translation problems with a data-driven, template-free sequence-to-sequence model. They tracked which starting materials were actual reactants, distinguishing them from other reagents like solvents or catalysts, and used the regex to uniquely tokenize recurring reagents, as their atoms were not mapped to products in the core reaction.

In 2019, \citet{Schwaller2019-lc} first applied a transformer for synthesis prediction, framing the task as translating reactants and reagents into the final product. Their model inferred correlations between chemical motifs in reactants, reagents, and products in the dataset (USPTO-MIT,\cite{jin_predicting_2017} USPTO-LEF, \cite{bradshaw_generative_2019} USPTO-STEREO\cite{schwaller_found_2018}). It required no handcrafted rules and accurately predicted subtle chemical transformations, outperforming all prior algorithms on a common benchmark dataset. The model handled inputs without a reactant-reagent split, following their previous work,\cite{schwaller_found_2018} and accounted for stereochemistry, making it valuable for universal application.
Then, in 2020, for automated retrosynthesis, \citet{schwaller_predicting_2020} developed an advanced Molecular Transformer model with a hyper-graph exploration strategy. The model set a standard for predicting reactants and other entities, evaluated with four new metrics: coverage, class diversity, round-trip accuracy, and Jensen–Shannon divergence. Constructed dynamically, the hypergraph allowed for efficient expansion based on Bayesian-like probabilities, showing high performance despite training data limitations. Notably, accuracy was improved after the re-synthesis of the target product from the newly generated molecular precursors was included in the model. This round-trip accuracy concept was also used by \citet{chen_deep_2021} and \citet{westerlund_chemformers_2024}. Also in 2020, \citet{zheng_predicting_2020} developed a "template-free self-corrected retrosynthesis predictor" (SCROP) using transformer networks and a neural network-based syntax corrector, achieving 59.0\% accuracy on a benchmark dataset.\cite{lowe_extraction_2012, schneider-2016-fingerprint} This approach outperformed other deep learning methods by over 2\% and template-based methods by over 6\%.

We now highlight advancements in synthesis prediction using the BART Encoder-Decoder architecture, including Chemformer by \citet{irwin_chemformer_2022}. This paper emphasized the computational expense of training transformers on SMILES and the importance of pretraining for efficiency. It showed that models pre-trained on task-specific datasets or using only the encoder stack were limited for sequence-to-sequence tasks. After transfer learning, Chemformer achieved state-of-the-art results in both sequence-to-sequence synthesis tasks and discriminative tasks, such as optimizing molecular structures for specific properties. They studied the effects of small changes on molecular properties using pairs of molecules from the ChEMBL database\cite{Gaulton2012-og} with a single structural modification. Chemformer’s performance was tested on the ESOL, Lipophilicity, and Free Solvation datasets.\cite{wu_moleculenet_2018} \citet{irwin_chemformer_2022} also described their use of an in-house property prediction model, but when models train on calculated data for ease of access and uniformity, they abstract away from real-world chemical properties. We again emphasize the importance of incorporating experimentally derived data into Chemistry LLM research to create more robust and relevant models. Continuously curating new, relevant datasets that better represent real-world chemical complexities will enhance the applicability and transferability of these models.

In 2023, \citet{Toniato2023-in} also applied LLMs to single-step retrosynthesis as a translation problem, but increased retrosynthesis prediction diversity by adding classification tokens, or "prompt tokens," to the target molecule's language representation, guiding the model towards different disconnection strategies. Increased prediction diversity has high value by providing out-of-the-box synthetic strategies to complement the human chemist’s work.
To measure retrosynthesis accuracy, \citet{li_retro-bleu_2024} introduced Retro-BLEU, a metric adapted from the BLEU score used in machine translation.\cite{Papineni2002-le} Despite progress in computer-assisted synthesis planning (CASP), not all generated routes are chemically feasible due to steps like protection and deprotection needed for product formation. Widely accepted NLP metrics like BLEU\cite{Papineni2002-le} and ROUGE\cite{Lin2004-md} focus on precision and recall by computing n-gram overlaps between generated and reference texts. Similarly, in retrosynthesis, reactant-product pairs can be treated as overlapping bigrams. Retro-BLEU uses a modified BLEU score, emphasizing precision over recall, as there is no absolute best route for retrosynthesis. Although not yet applied to LLM-based predictions, this approach has value by allowing future performance comparison with a single standard.

Finally, by expanding the use of encoder-decoder architectures outside synthesis prediction into molecular generation, \citet{Fang2023-ty} introduced MOLGEN, a BART-based pre-trained molecular language model, in a 2023 preprint updated in 2024. MOLGEN addressed three key challenges: generating valid SMILES strings, avoiding an observed bias that existed against natural product-like molecules, and preventing hallucinations of molecules that didn't retain the intended properties. Pre-trained on 100 million molecules using SELFIES\cite{krenn_self-referencing_2020} and a masked language model approach, MOLGEN predicts missing tokens to internalize chemical grammar. An additional highlight of this work is how MOLGEN uses "domain-agnostic molecular prefix tuning." This technique integrates domain knowledge directly into the model's attention mechanisms by adding molecule-specific prefixes, trained simultaneously with the main model across various molecular domains. The model's parameters would thus be adjusted to better capture the complexities and diversities of molecular structures, and domain-specific insights would be seamlessly integrated. To prevent molecular hallucinations, MOLGEN employs a chemical feedback mechanism, to autonomously evaluate generated molecules for appropriate properties, to guide learning and optimization. Such feedback foreshadows a core aspect of autonomous agents, which is their capacity for reflection. We will explore this further below.

\subsection{Multi-Modal LLMs}
Multitask or multimodal methods applied to chemistry are now described. In 2021, \citet{edwards-etal-2021-text2mol} proposed Text2Mol, which retrieved molecules using natural language descriptions as queries. This task required integrating both molecular and natural language modalities, making it a cross-lingual retrieval problem due to the distinct grammar of molecular representations. The researchers built a paired dataset of molecules with corresponding text descriptions, and developed an aligned semantic embedding space for retrieval. This was enhanced with a cross-modal attention-based model for explainability and reranking. One stated aim was to improve retrieval metrics, which would further advance the ability for machines to learn from chemical literature.
In their follow-up work in 2022, \citet{Edwards2022-yu} continued using SMILES string representations along with text descriptions. The two key applications were first, to generate captions for molecules from SMILES strings and second, to output molecules based on textual descriptions of desired properties.
With this in mind, several important challenges remain. First, molecules can have many possible descriptions based on their diverse properties. For example, aspirin can be described by its pain-relieving effects, its use in preventing heart attacks, its chemical structure (an ester and a carboxylic acid connected to a benzene ring in ortho geometry), or its degradation into salicylic acid and ethanoic acid in moist conditions \cite{carstensen_decomposition_1988}. Describing such a molecule therefore requires expertise in different chemistry domains, depending on its functions and properties. In contrast, image captioning for common objects like cats and dogs needs much less domain expertise. Thus, obtaining a large, paired dataset of chemical representations and textual descriptions is challenging. Another issue is that standard evaluation metrics, like BLEU, are inadequate for molecule-language tasks. To address this, \citet{Edwards2022-yu} developed MolT5, which pretrained a model on a large corpus of unlabeled natural language text and molecule strings using a denoising objective. They fine-tuned the model on gold standard annotations and improved the metric based on their prior Text2Mol work \cite{edwards-etal-2021-text2mol}. MolT5 effectively generated both molecule and caption outputs.

% \textcolor{blue}{The following is ok but may need to read better..it's a bit clunky. You also mentioned, Mayk, the Christofidelis paper as a good one and it currently only has a 1 line description}
%In 2021. \citet{edwards-etal-2021-text2mol} proposed Text2Mol, which retrieved molecules using natural language descriptions as queries. This task therefore required both the modalities of molecules and natural language to be integrated directly and so was seen as a cross-lingual retrieval problem, made difficult because the molecular representations had their own grammar.
%They built a paired dataset of molecules with corresponding text descriptions. An aligned semantic embedding space was developed for retrieval, enhanced with a cross-modal attention-based model for explainability and reranking. They also wanted to improve retrieval metrics, which would further advance the ability for machines to learn from chemical literature.
%In their second work from 2022, \cite{Edwards2022-yu} the two data modalities were, as would continue to be the typical SMILES string representation along with a text description. On the one hand, the SMILES string would be the input and a caption for the molecule would be the output. On the other hand, the authors described the benefits of inputting a textual description, perhaps based on needed properties and that molecule would be determined as an output.
%Yet there are some important challenges. First there are many possible descriptions for a molecule based on all the properties that same molecule might have. For example, an aspirin molecule could be described in terms of its pain-killing effects, its use to prevent heart-attacks, has it has both an ester and a carboxylic acid connected to a benzene ring with an ortho geometry, or how the aspirin may degrade in moist conditions to form salicylic acid and ethanoic acid.\cite{carstensen_decomposition_1988} Thus, different kinds of chemistry domain expert are required to describe aspirin depending on its many functions and many expected properties, which depend on its functional groups. In contrast, multi-modal captioning of images (images to text) containing cats and dogs relative to other household objects may require very little domain expertise. Hence, the first challenge is to obtain a large enough training dataset with matched pairs of chemical representations and textual descriptions. A second challenge is that typical evaluation metrics based on reference descriptions, such as BLEU, would fail to be able to adequately evaluate such molecule-language tasks. \citet{Edwards2022-yu} therefore took up the challenge of developing more molecule-text pairs. Their MolT5 first pretrained a model on a vast corpus of unlabeled natural language text and molecule strings using a denoising objective. They then fine tuned the pretrained model on certain gold standard annotations. They also built on the metric based on their prior Text2Mol work.\cite{edwards-etal-2021-text2mol} The MolT5-based models were able to effectively generate both molecule and caption outputs.

In other work, \citet{seidl_enhancing_2023} developed CLAMP. Trained on large biochemical datasets, CLAMP  adapts to new tasks using separate modules for chemical and language inputs, and predicts biochemical activity for drug discovery. \citet{xu_multilingual_2023} presented BioTranslator, a method for translating user-written text descriptions into non-text biological data, facilitating the discovery of novel cell types and applications in protein function prediction and drug target identification. This method enabled data exploration beyond controlled vocabularies using free text. ChatDrug, by \citet{liu_chatgpt-powered_2023}, integrates multimodal capabilities through a prompt module, a retrieval and domain feedback module, and a conversation module for systematic drug editing. It identifies and manipulates molecular structures for better interpretability in pharmaceutical research. \citet{Christofidellis2023-ea} introduced a multi-domain, multi-task language model capable of handling tasks across chemical and natural language domains without specific pretraining for each. \citet{liu_molxpt_2023} developed MolXPT, a unified model that integrates text and molecules for enhanced molecular property prediction and translation, demonstrating robust zero-shot molecular generation capabilities. \citet{zhang_pre-trained_2024} introduced PremuNet, a pre-trained multi-representation fusion network that enhances molecular property prediction by integrating various molecular data representations. \citet{Liu_2024_gitmol} developed GIT-Mol, integrating graph, image, and text data, significantly improving molecular property prediction and molecule generation validity. \citet{gao_dockingga_2024} advanced targeted molecule generation with DockingGA, combining transformer neural networks with genetic algorithms and docking simulations for optimal molecule generation, utilizing Self-referencing Chemical Structure Strings to represent and optimize molecules. \citet{zhou_instruction_2024} developed TSMMG, a teacher-student LLM for multi-constraint molecular generation, learning from a large set of text-molecule pairs and generating molecules that meet complex property requirements. \citet{zhu_3m-diffusion_2024} proposed 3M-Diffusion, a multi-modal molecular graph generation method that uses natural language descriptions to generate diverse, novel molecular graphs. \citet{gong_text-guided_2024} introduced TGM-DLM, a diffusion model for text-guided molecule generation that overcomes limitations of autoregressive models in generating precise molecules from textual descriptions. \citet{fang_moltc_2024} developed MolTC, a multimodal framework that effectively integrates graphical information of molecules for improved prediction of molecular interactions. \citet{ock_catalyst_2023} introduced CatBERTa, a model using textual inputs for predicting catalyst energies, demonstrating its potential to replace graph-based models and uncovering complex feature-property relationships. \citet{soares_beyond_2023} describe MULTIMODAL-MOLFORMER, a multimodal language model that predicts molecular properties by integrating chemical language representations with physicochemical features. It uses a causal multistage feature selection method to identify physicochemical features directly impacting target properties. These features are combined with molecular embeddings from MOLFORMER\cite{Ross2022-yp}, significantly enhancing prediction accuracy for complex tasks like biodegradability and PFAS toxicity.

%Other work on multi modality models followed up this early work. \citet{seidl_enhancing_2023} developed an activity prediction model (CLAMP) that adapted to new tasks using separate modules for chemical and language inputs, enhancing predictive performance in drug discovery. CLAMP was trained on large biochemical datasets, and showed improved performance on few-shot and zero-shot learning tasks. \citet{xu_multilingual_2023} presented BioTranslator, a multilingual translation method, which translates user-written text descriptions into non-text biological data, enabling the discovery of novel cell types and applications in protein function prediction and drug target identification. This took data exploration beyond controlled vocabularies using free text. \citet{liu_chatgpt-powered_2023} proposed ChatDrug, which integrates multimodal capabilities through a prompt module, a retrieval and domain feedback module, and a conversation module for systematic drug editing. It thus identifies and manipulates molecular structures for drug editing and better interpretability in pharmaceutical research. \citet{Christofidellis2023-ea} introduced a multi-domain, multi-task language model capable of handling tasks across chemical and natural language domains without specific pretraining for each. \citet{liu_molxpt_2023} developed MolXPT, a unified model that integrates text and molecules for enhanced molecular property prediction and translation, demonstrating robust zero-shot molecular generation capabilities. \citet{zhang_pre-trained_2024} introduced PremuNet, a pre-trained multi-representation fusion network that enhances molecular property prediction by integrating various molecular data representations. \citet{Liu_2024_gitmol} Developed GIT-Mol, integrating graph, image, and text data, which significantly improved molecular property prediction and molecule generation validity. \citet{gao_dockingga_2024} advanced targeted molecule generation with DockingGA, combining transformer neural networks with genetic algorithms and docking simulations for optimal molecule generation, utilizing Self-referencing Chemical Structure Strings to represent and optimize molecules. \citet{zhou_instruction_2024} developed TSMMG, a teacher-student LLM for multi-constraint molecular generation, learning from a large set of text-molecule pairs and generating molecules that meet complex property requirements. \citet{zhu_3m-diffusion_2024} Proposed 3M-Diffusion, a multi-modal molecular graph generation method that uses natural language descriptions to generate diverse, novel molecular graphs. \citet{gong_text-guided_2024} introduced TGM-DLM, a diffusion model for text-guided molecule generation that overcomes limitations of autoregressive models in generating precise molecules from textual descriptions. \citet{fang_moltc_2024} developed MolTC, a multimodal framework that effectively integrates graphical information of molecules for improved prediction of molecular interactions. \citet{ock_catalyst_2023} introduced CatBERTa, a model that uses textual inputs for predicting catalyst energies, demonstrating its potential to replace graph-based models and uncovering complex feature-property relationships. \citet{soares_beyond_2023} describe MULTIMODAL-MOLFORMER, a multimodal language model that predicts molecular properties by integrating chemical language representations with physicochemical features. It uses a causal multistage feature selection method to identify physicochemical features that have a direct impact on target properties. These features are combined with molecular embeddings from MOLFORMER\cite{Ross2022-yp}, significantly enhancing prediction accuracy for complex tasks like biodegradability and PFAS toxicity compared to current models. 

\subsection{Textual scientific LLMs}

LLMs are large deep neural network models. Therefore, their superior performance against other smaller models in classical machine learning tasks is somewhat expected.
Addressing tasks that seemed impossible to tackle in the past better illustrates LLM's outstanding capabilities.
That is, despite accurately predicting properties given well-structured information such as molecular features and descriptors, LLMs can access less structured data and extract information from simple natural language.
For instance, instead of developing a restricted representation, \citet{Huang2019-gw} used clinical annotations from the MIMIC-III\cite{mimic-iii} dataset to predict patient readmission. ClinicalBERT implements a pre-trained BERT architecture using a combination of masked language modeling and next-sentence prediction training schemes followed by supervised fine-tuning on readmission prediction.
Or, instead of pretraining, \citet{Zhao2024-hi} fine-tuned LLaMA on epilepsy data using an instruction-following approach to create EpilepsyLLM.
%
Similarly, SciBERT\cite{Beltagy2019-ri} and ScholarBERT\cite{Hong2022-mv} adapted BERT to scientific literature. 
\citet{Beltagy2019-ri} created a tokenizer specific for scientific texts extracted from scientific articles from semantic scholar\cite{Kinney2023-fj} and showed that SciBERT outperforms fine-tuned \texttt{BERT-base}\cite{Devlin2018-nl} in every task investigated. It shows that vocabulary quality plays an important role in the model's performance.
A few years later, \citet{Hong2022-mv} pre-trained BERT using RoBERTa\cite{Liu2019-ur} optimizations to improve pretraining performance. ScholarBERT was pre-trained on scientific articles from \texttt{Public.Resource.Org, Inc} and further fine-tuned on the tasks used for evaluation.
Despite using a much larger dataset, ScholarBERT did not outperform other LLMs trained with narrower domain datasets. Even against SciBERT, another LLM trained on multi-domain articles, ScholarBERT could not perform relatively better in tasks from biomedical, computer science, and material domains. However, ScholarBERT showed significant improvement in the ScienceExamCER\cite{Smith2019-vu} dataset, which contains semantic class annotations in a training corpus of 3rd to 9th grade science exam questions for named entity recognition (NER) tasks.

On the other hand, instead of pretraining LLMs on a large domain scope, models focused on only one field were also developed.
\citet{Guo2022-kr} argue that manually curating structured datasets is a sub-optimal, time-consuming, and labor-intensive task. Therefore, they automated data extraction and annotation from scientific papers using \texttt{ChemDataExtractor}\cite{Swain2016-se} and their in-house annotation tool\cite{MTurk}. 
ChemBERT\cite{Guo2022-kr} was pre-trained using a BERT model to encode chemical reaction information, followed by fine-tuning a NER head. ChemBERT outperformed other models such as BERT\cite{Devlin2018-nl} and BioBERT\cite{Lee2020-vl} in the product extraction task, presenting an improvement of $\sim$~6\% in precision. For the product role labeling task -- given the extracted compound, which role does it play in the reaction? --, it increases precision in $\sim$~5\% when compared to the same models.
The increase in performance might be due to training in a narrower domain, which allows the model to learn specific traits from the data instead of being more generalist. 
MatSciBERT\cite{Gupta2022-hy} and MaterialsBERT\cite{Shetty2023-ew} followed a similar strategy. 
\citet{Gupta2022-hy} developed MatSciBERT by fine-tuning SciBERT\cite{Beltagy2019-ri} on the Material Science Corpus (MSC), their curated dataset focused on materials extracted from Elsevier's scientific papers. MatSciBERT shows an accuracy improvement of $\sim$~3\% compared to SciBERT on classifying an article subject based on its abstract.
Differently, MaterialsBERT\cite{Shetty2023-ew} fine-tuned PubMedBERT\cite{Gu2021-yn} on 2.4M abstracts extracted from material science articles using a masked training approach. MaterialsBERT was then used to generate a contextual encoded representation of the abstract to train a named entity relationship (NER) model. Reporting an increase in precision on their test dataset of $\sim$~1\%, $\sim$~2\%, and $\sim$~10\% for PubMedBERT, MatBERT, and ChemBERT, respectively.

Considerable effort was also employed to develop such models focused on biology tasks.
They follow a similar trend of training an LLM model on a large training corpus like Wikipedia, scientific data extracted from a scientific database, and textbooks, followed by fine-tuning specific downstream tasks.
\citet{Shin2020-cp} pre-trained different Megatron-LM\cite{Shoeybi2019-hr}, another BERT-like LLM, models with different sizes, originating the BioMegatron family of models. Considering models with 345M, 800M, and 1.2B parameters and vocabularies with 30k and 50k tokens, they compared the influence of model size on its performance. These models were pre-trained using abstracts from the PubMed dataset and full-text scientific articles from PubMed Central (PMC), similar to BioBERT\cite{Lee2020-vl}. The largest 1.2B training started from a \texttt{BERT-uncased} checkpoint to save time. Surprisingly, the largest model did not perform better than the smaller ones. In fact, the 345M parameters using the 50k tokens vocabulary consistently outperformed other models in NER and relation extraction (RE) tasks. Interestingly, the model size seems relevant for the SQuAD\cite{Rajpurkar2016-og} dataset, showing that LLMs trained on small, domain-specific datasets may lack generalization abilities.
%
BioBERT\cite{Lee2020-vl} used data from Wikipedia, textbooks, PubMed abstracts, and PMC full-text corpus to pretrain a BERT architecture. Outperforming the original BERT in all benchmarks tested and even SOTA models in some benchmarks (NCBI disease, 2010 i2b2/VA, BC5CDR, BC4CHEMD, BC2GM, JNLPBA, LINNAEUS, Species-800).
\citet{Peng2020-bp} developed a multi-task BERT evaluated on the BLUE\cite{Peng2019-yb} benchmark called BlueBERT. The model was pre-trained on PubMed abstracts and MIMIC-III\cite{mimic-iii} and fine-tuned on BLUE tasks, achieving similar results as BioBERT in multiple benchmarks.
PubMedBERT\cite{Gu2021-yn}, following the approach adopted in SciBERT, developed a domain-specific vocabulary. They used 14M abstracts extracted from PubChem to pre-train PubMedBERT. In addition, they curated and grouped multiple biomedical datasets to develop BLURB, their comprehensive benchmark for biomedical NLP tasks, such as NER, sentence similarity, document classification, and question-answering. \citet{Gu2021-yn} showed that PubMedChem considerably outperformed other LLMs in the BLURB benchmark, mainly in PubMedQA and BioQSA datasets. The second best-evaluated model in these datasets was BioBERT, evidencing the importance of domain-specific knowledge to high-performance LLMs.

The models discussed previously in the section use an encoder-only LLM to encode information from scientific data. The learned encoded representation is then further used to make predictions by feeding it to simpler models. A different approach involves training a decoder model. Using a decoder model aims to address the lack of generation ability of the encoder-only models. By implementing a decoder, the model can address a different group of generative tasks, such as question-answering and document classification, using generated labels instead of following a pre-defined set of possible classes.
%
Darwin\cite{Xie2023-nh} aims to create domain-specific LLMs for natural science by first fine-tuning LLaMA-7B on FAIR, a general Question-Answering (QA) dataset, and then fine-tuning it on scientific QA datasets. Scientific QA instructions were obtained from SciQ\cite{Welbl2017-jv} and generated by the authors using the Scientific Instruction Generation (SIG) model also developed by the authors. Their SIG model is fine-tuned from Vicuna-7B to convert full-text scientific papers into a set of QA pairs. This approach presented an improved performance of DARWIN in several regression and classification benchmarks. Interestingly, Using LLaMA-7B fine-tuned on FAIR only -- with no scientific-specific QA fine-tuning -- led to similar results in six out of nine benchmarks with metrics available for both models. 

In biology, BioGPT\cite{Luo2022-sv} pre-trained a GPT-2 model architecture using 15M abstracts from PubChem corpus. BioGPT was evaluated on four tasks across five benchmarks: end-to-end relation extraction on BC5CDR, KD-DTI, and DDI, question answering on PubMedQA, document classification on HoC, and text generation on the previously listed benchmarks. fine-tuning BioGPT on downstream tasks (except text generation) showed its superiority against other encoder-only LLMs in the biomedical domain, such as BioBERT and PubMedBERT. Focusing on text generation, the authors qualitatively compared BioGPT and GPT-2 generations. They conclude that BioGPT demonstrates better text generation. However, no metric was used, making the comparison difficult to measure.
%
With a similar idea, \citet{Wu2023-tb} first pre-trained an LLaMA2 model with the MedC-k dataset, consisting of 4.8M academic papers and 30K textbooks. In the sequence, the model was aligned through instruction tuning using the MedC-I dataset, a set of medical QA problems. PMC-LLaMA\cite{Wu2023-tb} outperforms LLaMa-2 and ChatGPT in multiple biomedical QA benchmarks despite its size $\sim$~10 times smaller. Interestingly, the authors show that the performance of PMC-LLaMA on MedQA\cite{Jin2020-he}, MedMCQA\cite{Pal2022-te}, and PubMedQA\cite{Jin2019-uw} benchmarks progressively increases as more knowledge is injected, the model size is increased, and more instructions are included in instruction tuning. 
%
% BioMedGPT-LM\cite{Luo2023-gw}
% %
% LLaVa-Med\cite{}
% %
% BioMedLM\cite{}
% %
% MatGPT\cite{}
% %
% MediSwift\cite{}
% %
% %
% CheXagent\cite{}
% %
% BioMistral\cite{}
% \todo{add other more recent studies.}

% \todo{
% Discuss DSPY\cite{Khattab2023-io}
% }

\subsection{The use of ChatGPT in Chemistry}

With the rise of ChatGPT, we review here how many researchers have wanted to test the capability of such an accessible decoder-only LLM. \citet{castro_nascimento_large_2023} wrote the first notable paper on ChatGPT's impact on Chemistry. The authors emphasize that LLMs, trained on extensive, uncurated datasets potentially containing errors or secondary sources, may include inaccuracies limiting their ability to predict chemical properties or trends. The paper highlighted that while LLMs could generate seemingly valid responses, they lacked true reasoning or comprehension abilities and would perpetuate existing errors from their training data. However, the authors suggested that these limitations could be addressed in the future.
The work serves as a benchmark to qualitatively assess improvements in generative pre-trained transformers. For example, five tasks were given to ChatGPT (GPT-3). The accuracy for converting compound names to SMILES representations and vice versa was about 27\%, with issues in differentiating alkanes and alkenes, benzene and cyclohexene, or \textit{cis} and \textit{trans} isomers. ChatGPT found reasonable octanol-water partition coefficients with a 31\% mean relative error, and a 58\% hit rate for coordination compounds' structural information. It had a 100\% hit rate for polymer water solubility and a 60\% hit rate for molecular point groups. Understandably, the best accuracies were achieved with widely recognized topics. The authors concluded that neither experimental nor computational chemists should fear the development of LLMs, nor task automation. Instead, they encouraged the improvement of dedicated AI tools for specific problems, with their integration into research, as facilitators.


The sole use of ChatGPT for chemistry and any apparent advancement in chemistry seems somewhat limited. \citet{humphry_potential_2023}, \citet{emenike_was_2023}, and \citet{fergus_evaluating_2023} address the use of ChatGPT in chemical education. There are also a few papers that describe the use of ChatGPT on a specific area of chemical research,\cite{zheng_shaping_2023, zheng_chatgpt_2023, zheng_gpt-4_2023}  where fine-tuned GPT models are used to direct the synthesis and functional optimization of Metal Organic Framewoks (MOFs), merging computational modeling with empirical chemistry research. 
\citet{deb2024-uc} provide a thorough assessment of ChatGPT's effectiveness in material science through various tasks in computational material science, though the perspective is subjective. ChatGPT assisted in computational materials science by providing crystal space groups for simple compounds, suggesting inputs for simulations, refining analysis with specific rules, and identifying resources. The authors highlight ChatGPT's potential to write code for enhancing processes and as a tool for those without prior expertise, particularly in catalyst development for CO2 capture.
We highlight three points about using ChatGPT alone. First, reliable outputs require detailed and accurate input, as \citet{deb2024-uc} showed, where ChatGPT struggled to mine or predict crystal structures. Second, standardized methods for reproducing and evaluating GPT work are still unclear. Third, this work naturally leads to the inference that additional chemical tools or agents are needed to achieve more complex thinking, as described by Bloom’s Taxonomy.\cite{bloom1968taxonomy,bloom2010taxonomy}
Bloom’s taxonomy categorizes educational goals into hierarchical levels: Remembering, Understanding, Applying, Analyzing, Evaluating, and Creating. Remembering involves recalling facts, Understanding means restating a concept, and Applying uses a theory in a new situation. Analyzing breaks down a mechanism into parts to understand connections and differences. Evaluating involves making value judgments, and Creating entails building new structures from diverse elements.
Currently, Large Language Models (LLMs) and Autonomous Agents are limited in replicating higher-level thinking compared to human understanding. To better quantify their capabilities in this area, we therefore recommend adopting a quality metric based on Bloom’s taxonomy. This educational framework can serve as an effective tool for evaluating the sophistication of LLMs and autonomous agents, especially when tackling complex chemical challenges. Bloom's taxonomy would thereby provide a structured approach to assess higher-order thinking and reasoning.

\subsubsection{Automation}

The evolution of artificial intelligence in chemistry has fueled the potential for automating scientific processes. For example, in 2019, \citet{coley_robotic_2019} developed a flow-based synthesis robot proposing synthetic routes and assembling flow reaction systems, tested on medically relevant molecules, and in 2020, \citet{gromski_universal_2020} provided a useful exploration on how chemical robots could outperform humans when executing chemical reactions and analyses. They developed the Chemputer, a programmable batch synthesis robot handling reactions like peptide synthesis and Suzuki coupling. In 2021, \citet{grisoni_combining_2021} combined deep learning-based molecular generation with on-chip synthesis and testing. The Automated Chemical Design (ACD) framework by \citet{goldman_defining_2022} provides a useful taxonomy for automation and experimental integration levels.
Thus, automation promises to enhance productivity through increased efficiency, error reduction, and the ability to handle complex problems, as described in several excellent reviews regarding automation in chemistry,\cite{schneider_automating_2018, janet_artificial_2023, coley_autonomous_2020, coley_autonomous_2020-1,thakkar_artificial_2021, shen_automation_2021, liu_microfluidics_2021} This increased productivity may be the only possible approach to exploring the vastness of all chemical space. 
To fully leverage AI in property prediction, inverse deisgn and synthesis prediction, it must be integrated with automated synthesis, purification, and testing. This automation should be high-throughput, 24/7, and driven by AI-based autonomous decision-making (sometimes called ``lights-out'' automation). \citet{janet_artificial_2023} highlighted challenges in multi-step reactions with intermediate purifications, quantifying uncertainty, and the need for standardized recipe formats. They also stated the limitations of automated decision-making.
Other limitations exist like the restriction of machines to pre-defined instructions, an inability to originate new materials, and lower likelihood of serendipitous discoveries. Yet, when dedicated tools can be connected together to address each step of an automated chemical design, then these limitations can be systematically addressed through advancements in LLMs and Autonomous agents, discussed in the next section.

\section{LLM-based autonomous agents}\label{sec:agents}

The term ``agent'' originates in philosophy, referring to entities capable of making decisions\cite{Salamon2011-lz}. Hence, in artificial intelligence, an ``agent'' is a system that can perceive its environment, make decisions, and act upon them in response to external stimuli\cite{Xi2023-ee}. As described above, language has enabled humans to decide and act to make progress in response to the environment and its stimuli, and so LLMs are naturally ideal for serving as the core of autonomous agents. Thus, in agreement with \citet{Gao2024-zp}, we define "language agents" as a model or program (typically based on LLMs) that receives an observation from its environment and executes an action in this environment. Here, environment means a set of tools and a task.
Hence, "LLM-based autonomous agents" refer to language agents whose core is based on an LLM model.
%LLMs are therefore the prime candidates to act as the core of autonomous agents because of the substantial advancements in their ability to understand human language. Hence, ``LLM-based autonomous agents'' retain an LLM core that is their main component, and from now on, whenever the term ``agent'' is used, it is implied that an LLM is at the core.
Comprehensive analyses of these agents are available in the literature\cite{Wang2023-kc, Xi2023-ee, Gao2024-zp}, but this section highlights key aspects to prepare the reader for future discussions.
% For the reader interested in implementing these ideas in your workflow, we strongly suggest a deeper understatement of what agents are before applying them to your problem.

There is no agreed definition of the nomenclature to be used to discuss agents.
For instance, \citet{Gao2024-zp} created a classification scheme that aims to group agents by their autonomy in biological research. This means a level 0 agent has no autonomy and can only be used as a tool, while a level 3 agent can independently create hypotheses, design experiments, and reason.
%
Another previously suggested framework highlights agents' construction, application, and evaluation as a parallel between agents and neural networks. 
% The construction phase involves selecting an architecture and enabling task-specific functionalities, similar to choosing a neural network's design and tuning its parameters for specific goals.
Following this perspective, \citet{Wang2023-kc} categorizes agent components into four modules: profiling, memory, planning, and action. In contrast, \citet{Weng2023-ic} also identifies four elements — memory, planning, action, and tools — but with a different emphasis. Meanwhile, \citet{Xi2023-ee} proposes a division into three components: brain, perception, and action, integrating profiling, memory, and planning within the brain component, where the brain is typically an LLM. 
%
Recently, \citet{Sumers2023-ct} proposed Cognitive Architectures for Language Agents (CoALA), a conceptual framework to generalize and ease the design of general-purpose cognitive language agents. In their framework, a larger cognitive architecture composed of modules and processes is defined. CoALA defines a memory, decision-making, and core processing module, in addition to an action space composed of both internal and external tools. While internal tools mainly interact with the memory to support decision-making, external tools compose the environment, as illustrated in Figure~\ref{fig:agents}.
Given a task that initiates the environment, the ``decision process'' runs continuously in a loop, receiving observations and executing actions until the task is completed. For more details, read Reference~[\citenum{Sumers2023-ct}].

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.99\textwidth]{figs/agents3.png}
    \caption{
    Agent's architecture as defined in this review. According to our definition, an agent is composed of a central program (typically an LLM and the code to implement the agent's dynamic behavior) and the agent modules. The agent continuously receives observations from the environment and decides which action should be executed to complete the task given to it. Here, we define the agent as the set of elements whose decision is trainable, that is, the LLM, the agent code, the decision process, and the agent modules. Given a task, the agent uses the agent modules (memory, reasoning, planning, profiling) and the LLM to decide which action should be executed. This action is executed by calling a tool from the environment. After the action is executed, an observation is produced and fed back to the agent. The agent can use perception to receive inputs in different modalities from the environment. A) Description of agent modules, B) illustration of the agent architecture, C) illustration of the environment components, D) description of tools elements present in the environment.
    }
    \label{fig:agents}
\end{figure}

In this review, we define autonomous agent systems as models (typically LLMs) that continuously receive observations and execute actions within an environment, as described by \citet{Gao2024-zp}. Nevertheless, in contrast to CoALA\cite{Gao2024-zp}, we will rename ``internal tools'' as ``agent modules'' and ``external tools'' simply as ``tools'', for clarity. The agent consists of trainable decision-making components such as the LLM itself, policy, memory, and reasoning scheme. In contrast, the environment comprises non-trainable elements like the task to be completed, API access, interfaces with self-driving labs, dataset access, and execution of external code. Referring to the former as agent modules emphasize their inclusion in the agent, while referring to the latter as tools highlight their role in the environment. We discuss five main types of actions. Among these five, memory, planning and reasoning, and profiling are agent modules, while tools are part of the environment. Because the perception is how the agent interacts with the environment, not a trainable decision, we decided to include it as part of the environment.
(Figure~\ref{fig:agents}):
(i)   memory,
(ii)  planning and reasoning,
(iii) profiling,
(iv)  perception, and
(v)   tools,

\subsection{Memory module}

Memory refers to the ability to store and recall information from past interactions and experiences to inform future decisions and actions. There are multiple types of memory in agents, namely sensory memory, short-term memory, and long-term memory. 
%
Sensory, or procedural,  memory is knowledge embedded into the model's parameters during pretraining and/or in heuristics implemented into the agent's code. 
%
Short-term, or working, memory includes the agent's finite knowledge during a task, incorporating interaction history and techniques like in-context learning\cite{Brown2020-ej}, which leverages the limited input's context length for information retention. 
%
Long-term memory involves storing information externally, typically through an embedded vector representation in an external database. In the original CoALA\cite{Gao2024-zp} paper, long-term memory is further divided into two different types of long-term memory: episodic, which registers previous experiences, and semantic, which stores general information about the world.

A major challenge in using agents is the limited context window, which restricts the amount of in-context information and can lead to information loss, thereby impacting the effectiveness of short-term and long-term memory. Solutions involve summarizing memory content\cite{Liang2023-in}, compressing memories into vectors\cite{Zhang2023-yw, Zhu2023-tx, Zhong2023-pa}, and utilizing vector databases\cite{Han2023-yf} or combinations thereof\cite{Zhao2023-ra}, with various databases available such as ChromaDB, FAISS, Pinecone, Weaviate, Annoy, and ScaNN.\cite{ANN-benchmark-eo} Addressing these challenges to enhance agent memory continues to be a significant area of research\cite{Hatalis2023-fh}.

\subsection{Planning and reasoning modules}
Planning involves identifying a sequence of actions designed to achieve a specified goal. In the context of language agents, this means generating steps or strategies that the model can follow to solve a problem or answer a question, which can be enhanced with retrieval from previous experiences\cite{Park2023-fr} and feedback from post-execution reasoning\cite{Raman2022-zo, Dhuliawala2023-wp}. 
%
Reasoning refers to the process of drawing conclusions or making decisions based on available information and logical steps. For example, there are studies that demonstrate the benefits of LLM reasoning for question answering, where new context tokens can be integrated in a step-by-step way to guide the model towards more accurate answers\cite{Huang2022-rs, Kojima2022-bd, Wei2022-rm, Wang2022-lq, Yao2022-db, Hao2023-ng}. One popular reasoning strategy is Chain-of-Thought (CoT),\cite{Wei2022-rm,Liu2023-zb, Yao2023-ph, Shinn2023-kt, Kang2023-ol, Qian2024-pi} which substantially boosts QA performance by generating intermediate reasoning steps. This reduces hallucinations and enhances interpretability, as demonstrated by improved results in models like PaLM\cite{Anil2023-ja} and GPT-3 with benchmarks like GSM8K\cite{Cobbe2021-ef}, SVAMPs\cite{Jie2022-fy}, and MAWPS\cite{Lan2021-as}.

Final tasks are often decomposed into intermediary ones using a cascading approach, similar to Zero-shot-CoT\cite{Kojima2022-bd} and RePrompt\cite{Raman2022-zo}. However, while CoT is considered as single-path reasoning, CoT extensions like Tree-of-Thoughts\cite{Yao2022-db}, Graph-of-Thoughts\cite{Besta2023-sd}, Self-consistent CoT\cite{Wang2022-lq}, and Algorithm-of-Thoughts\cite{Sel2023-vr} offer multi-path reasoning. Furthermore, other models have pitted multiple agents against each other to debate or discuss various reasoning paths,\cite{Liang2023-mz, Du2023-wj, Chan2023-qf} while others use external planners to create plans\cite{Song2022-uw, Liu2023-cp}. 
A feedback step during the execution of the plan was a further extension of the CoT ideas; this enables agents to refine their actions based on environmental responses adaptively, which is crucial for complex tasks.\cite{Madaan2023-kd, Xi2023-sj}

Another interesting reasoning scheme is the Chain-of-Verification(CoVe), \cite{Dhuliawala2023-wp} where once an answer is generated, another LLM is prompted to generate a set of verification questions to check for agreement between the original answer and the answers to the verification questions such that the final answer can be refined.
The ReAct\cite{Yao2022-db} -- Reason+Act -- model proposes adding an observation step after acting. This means the LLM first reasons about the task and determines the necessary step for its execution, it performs the action and then observes the action's result. Reasoning on that result, it can subsequently perform the following step. 
Similarly, Reflexion\cite{Shinn2023-kt} also implements a reasoning step after executing an action. However, Reflexion implements an evaluator and a self-reflection LLMs to not only reason about each step but also to evaluate the current trajectory the agent is following using a long-term memory module.

ReAct and Reflexion are closed-ended approaches where the agent starts with all the tools and must determine which to use. To address more open-world challenges, \citet{Wang2023-ni} introduced the Describe, Explain, Plan, and Select (DEPS) method, which extends this approach. Lastly, human inputs can also be used to provide feedback to the agent. Providing feedback using a human-in-the-loop approach is particularly interesting in fields where safety is a main concern.

\subsection{Profiling module}
Language agents can incorporate the profile through the LLM or through the agent code. Specifically, LLMs can be configured to perform in specific roles, such as coders, professors, students, and domain experts, through a process known as profiling. This approach involves inputting psychological characteristics to the agent, significantly impacting its decision-making process \citep{Deshpande2023-iz, Hong2023-ma, Li2023-uj, Jinxin2023-wp}. Profiling enables the creation of multi-agent systems that simulate societal interactions, with each agent embodying a unique persona within the group \citep{Park2023-fr, Qian2023-sd}. The most prevalent technique for profiling, called ``handcrafting'', requires manually defining the agent's profile, often through prompts or system messages \citep{Shao2023-ic, Ke2023-mp}. While profiling can also be automated with LLMs \citep{Wang2023-jq}, this method is suited for generating large numbers of agents but may offer less control over their overall behavior. An interesting application of profiling is the development of agent sets that reflect demographic distributions \citep{Argyle2023-gf}.

\subsection{Perception}
Perception is an analog to the human sensory system, which interprets multimodal information such as text, images, or auditory data, transforming it into a format comprehensible by LLMs, as demonstrated by SAM\cite{Kirillov2023-jc}, GPT4-V\cite{GPT4-v}, LLaVa\cite{Liu2023-op}, Fuyu8B\cite{FUYU8B-2023}, and BuboGPT\cite{Zhao2023-fn}. In our proposed architecture, the perception is responsible for converting the task and the observations to a data representation that can be understood by the agent. Moreover, advancements in LLMs have led to the development of even more versatile models, such as the any-to-any Next-GPT\cite{Wu2023-pw} and the any-to-text Macaw-LLM\cite{Lyu2023-sa}. Employing multimodal LLMs in decision-making processes can simplify perception tasks for agents, with several studies exploring their use in autonomous systems\cite{Wang2024-ct, Gao2023-gk}. 
% The application of visual object recognition techniques further enhances this approach.


\subsection{Tools}

In our proposed definition (see Figure \ref{fig:agents}b), tools or actions are part of the environment. The agent can interact with this environment by deciding which action to execute through the decision-making process. The set of all possible actions that can be selected is also known as the ``action space''. 

The decision process is composed by three main steps: proposal, evaluation, and selection. During the proposal, one or more action candidates are selected using reasoning\cite{Yao2022-db}, code structures\cite{Wang2023-os, Park2023-fr}, or simply by selecting every tool available\cite{Ahn2022-oa}.\cite{Huang2022-rs, Chen2021-vs, Wang2022-lq} The evaluation process consists of evaluating each selected action according to some metric to predict which action would bring more value to the agent. Lastly, the action is selected and executed.

Given that pre-trained parameters (sensory memory) are limited, the model must use tools for complex tasks in order to provide reliable answers.
However, LLMs need to learn how to interact with the action space and how and when to use those tools most accurately.\cite{Qin2023-ag} 
LLMs can be pre-trained or fine-tuned with examples of tool use, enabling them to operate tools and directly retrieve tool calls from sensory memory during a zero-shot generation.\cite{Nakano2021-od} Recent studies investigate this approach, particularly focusing on open-source LLMs.\cite{Schick2023-oe, Parisi2022-pj, Qian2023-oa} 

% Building on this, more powerful, high-performance foundational models, developed on vast amounts of data, can be utilized to understand how tools should be used. By analyzing tool usage, these foundational models can capture insights into more effective tool use, thereby generating datasets that may be used to fine-tune a smaller or open-source model, creating a domain-specific LLM capable of replicating tool-use and retrieval pattern for that specific domain.

As foundational AI models become more advanced, their abilities can be expanded. It was shown that general-purpose foundation models can reason and select tools even with no fine-tuning. For example, MRKL\cite{Karpas2022-uc} (pronounced ``miracle'') implements an extendable set of specialized tools known as neuro-symbolic modules (tools) and a smart "router" system to retrieve the best module based on the textual input. These neuro-symbolic modules are designed to handle specific tasks or types of information, equipped with built-in capabilities and task-relevant knowledge. This pre-specialization allows the model to perform domain-specific tasks without needing a separate, domain-specific dataset.
This design addresses the problem of LLMs lacking domain-specific knowledge and eliminates the need for the costly and time-consuming fine-tuning step with specialized data annotation.\citet{Chen2023-df}. The router can receive support from a reasoning strategy to help select the tools\cite{Chen2023-df} or follow a previously created plan\cite{Wang2023-ni}. Recent advances have shown that LLMs can develop new tools of their own\cite{Cai2023-ui, Qian2023-no, Yuan2023-xq}, enabling agents to operate, as needed, in dynamic and unpredictable ``open-worlds'', on unseen problems as illustrated by Voyager\cite{Wang2023-os}. This capability allows agents to evolve and improve continually.

\section{LLM-Based Autonomous Agents in Scientific Research}

The previous section introduced key concepts relevant to any description of the development of autonomous agents. Here, we now focus on which agents were developed for scientific purposes, and ultimately for chemistry. Previous sections of this review have discussed how LLMs could be powerful in addressing challenges in molecular property prediction, inverse design and synthesis prediction. When we consider the value of agents in chemistry and the ability to combine tools that, for example, search the internet for established synthetic procedures, look up experimental properties and control robotic synthesis and characterization systems, we can see how autonomous agents powerfully align with the broader theme of automation, which will lead to an acceleration of chemical research and application.

\begin{table*}[ht]
    \small
    \caption{\ Scientific LLM systems and agents. We identify the studies we classified as an agent with the icon \agent\cite{Hilmy-bot} and multi-agent systems with the icon \agent\agent. \W, \S, and \L\cite{Laisa-memory} mean the agent bases his behavior on sensory, short, and long memory components, respectively. Besides the textual capabilities of LLM-based agents, \audio\cite{Freepik-audio} means the agent has additional audio perception.
    % \textual, \view\cite{Kiranshastry-view}, and \audio\cite{Freepik-audio} mean the agent has textual, visual, and audio perception.
    }
    \label{tab:agents}
        \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}m{3.2cm}|cccm{6.5cm}c}
        Agent   & Memory & Planning & Reasoning & Action & Release \\\hline
        CRISPR-GPT\cite{Huang2024-pg}\agent\agent
        &\S   &\c & \c  & Tool for gene editing experiments design & 2024.04\\
        TAIS\cite{Liu2024-xm}\agent\agent
        &\S   &\c & \c  & Tools for gene expression data analysis  & 2024.02\\
        SciAgent\cite{Ma2024-no}\agent
        &\W\L   &\c & \c  & Trained Mistral for tool usage. Evaluated it using MathToolBench's tools & 2024.02\\
        STORM\cite{Shao2024-qk}
        &\S\L   &\c &\c  & Article writing using retrieval from multi-LLM conversations and pre-generated outline & 2024.02\\
        \citet{Volker2024-nv}
        &\S     &   &   & Regression with ICL and text retrieval  & 2024.02\\
        ProtAgent\cite{Ghafarollahi2024-kj} \agent\agent
        &\S\L   & \c & \c & Tools for proteins information retrieval, analyzing, \textit{de novo} design, and 3D folded structure generation & 2024.01\\
        PaperQA\cite{Lala2023-ru}\agent
        &\S\L   &\c &\c & Tools to search the scientific literature, gather evidence, and answer questions   & 2023.12\\
        WikiCrow\cite{wikicrow2024}\agent          
        &\S\L   &\c &\c & Uses PaperQA as a tool & 2023.12\\
        Coscientist\cite{Boiko2023-ot}\agent     
        &\S     &\c &\c & Tools for running Python code, web-searching, and interacting with lab equipment & 2023.12\\
        Eunomia\cite{Ansari2023-qi}\agent
        &\S     &   &\c & Tools for literature and dataset searching and a chain-of--verification loop & 2023.12\\
        CALMS\cite{Prince2023-ar}\agent
        &\L     &   &   & Tools for using the Materials Project API, designing experiments, and using a hardware API to perform the experiment  & 2023.12\\
        CoQuest\cite{Liu2023-ye}\agent
        &\S & & \c & & 2023.10\\
        eXpertAI\cite{Wellawatte2023-rw}\agent
        &\S     &   &\c & Tools for applying XAI methods & 2023.11\\
        BioPlanner\cite{ODonoghue2023-tx}\agent
        &\S     &\c &\c & Tool for protocol searching in the BioProt dataset  & 2023.10\\
        IBM ChatChem\cite{Janakarajan2023-fk}\agent
        &\S     &   &   & Tools for cheminformatics and accessing GT4SD and HuggingFace models & 2023.09\\
        ChatMOF\cite{Kang2023-zs}\agent
        &\W\S   &   & \c  & Tools for database search, property prediction, and MOF's structure generation & 2023.08\\
        i-Digest\cite{Mourino2023-fj} \audio
        &\S     &   &   & Uses the whisper model to process audio transcription from classes and write summaries and following up questions  & 2023.06\\
        BOLLaMa \cite{Rankovic2023-bd}          
        &\W     &   &   & Implements an LLM interface to ease the usage of their BO code & 2023.06\\
        text2concrete\cite{Kruschwitz2023-da}   
        &\S     &   &   & Uses ICL to predict compressive strength from concrete formulation  & 2023.06\\
        MAPI\_LLM\cite{Ramos2023-ps}\agent
        &\S\L   &   &\c &Database access and LLM prediction using ICL& 2023.06\\
        BO-LIFT\cite{Ramos2023-cs}              
        &\S     &   &   &Regression using ICL and text retrieval & 2023.04\\
        ChemCrow\cite{Bran2023-jk}\agent
        &\S     &   &\c & Molecular, cheminformatics, search and critique tools & 2023.04 \\
    \end{tabular*}
\end{table*}

%Previous studies have illustrated the high potential for natural language processing models in chemistry.
%As described above,
It was \citet{Hocky2021-mr} who discussed the early stages of models that could automate programming and, hence, the expected impacts in chemistry.
%that we are now witnessing.
Then, early work by \citet{White2023-bi} applied LLMs that could generate code to a benchmark set of chemical problems. In that case, not only were LLMs demonstrated to possess a notable understanding of chemistry, based on accurate question answering, but \citet{White2023-bi} imagined a potential to use them as base models to control knowledge augmentation and a variety of other tools. Thus, these LLMs could be used to execute routine tasks, optimize procedures, and enhance the retrieval of information from scientific literature across a range of scientific domains. To the best of our knowledge, this is the first review of autonomous agents in chemistry that have evolved since these two visionary conceptual perspectives. A deeper exploration follows below.
One driving motivation for the need to augment LLMs with a more pertinent and dedicated knowledge base is the need to circumvent problems of a limited context prompt window, and the restriction that once an LLM is trained, any new information is beyond it's reach since it necessarily has fallen outside its corpus of training data. Furthermore, LLMs are also known to hallucinate. Their predictions are probabilistic and, in science, if experimental evidence is available, then there is great value in building from known domain-specific information. Some improved prompt engineering can aid in the generation of results that are more likely to be accurate, but the use of autonomous agents may solve such problems completely in this next phase of AI in chemistry.
%LLMs' knowledge is constrained by their training data, exemplified in that any fact dated after the model is trained, is inaccessible to the model. A direct consequence is that LLMs cannot generate up-to-date information, they fail to give accurate domain-specific information, and they often hallucinate nonexistent scientific papers. Even though common prompt-answering schemes cannot solve these problems, they can be addressed by implementing autonomous agent components as discussed in Section \ref{sec:agents}. 
In fact, even adding one or two components when building an agent, as opposed to a whole suite, has shown some significant gains.
%Interestingly, some studies have implemented only some components instead of an entire agent and still have shown how these components individually can impact scientific research.
% For example, \citet{Ramos2023-cs} used in-context learning and a long-term memory component to show improvement in property predictions even past the window context limitation describved above. \citet{Volker2024-nv} also used short-term memory to provide domain-specific knowledge to the LLM. Using other components, \citet{Ouyang2023-qd} structured a prompt to guide the model through a logical sequence of reasoning with CoT to improve the LLM's ability to both answer chemistry questions from SciBench\cite{Wang2023-bp} and generate chemical formulas.

%LLMs were shown to have potential as central models for more complex LLM applications.
Building on this foundation, \citet{Ramos2023-cs} illustrated that LLMs could directly predict experimental outcomes from natural language descriptions, a technique they incorporated into a Bayesian optimization (BO) algorithm to streamline chemical processes. Because in-context learning was used, their approach did not require additional model training or finetuning, thereby greatly simplifying the optimization algorithm.
\citet{Rankovic2023-ge} also explored BO using natural language. They used an LLM to encode chemical reaction procedures, described using natural language, and then trained a multi-layer perceptron (MLP) head to predict the reaction yield from the latent encoded representation of the procedure. This effective transfer-learning approach minimized training time by keeping the LLM frozen while updating only the MLP. Extending these ideas, \citet{Volker2024-nv} suggested sampling multiple model completions and adding a verifier model to select the next best procedure to continue the BO algorithm. They also used in-context learning and a short-term memory component to optimize alkali-activated concrete mix design. The authors thus underscored how augmenting with knowledge-driven design can outperform traditional data-driven design. These are examples of how agent-based approaches can execute complex optimization algorithms in a step-by-step approach, directly contributing to automation and leading to faster and more efficient experimental design.

To better promote new ideas regarding AI in scientific research, \citet{Jablonka2023-ng} organized a hackathon in March 2023.
During this one-day hackathon, 14 innovative projects were developed to address chemical problems centered around predictive modeling, automation, knowledge extraction, and education. We below highlight agent-based approaches from that Hackathon. First, MAPI\_LLM\cite{Ramos2023-ps} is an agent with access to the Materials Project API (MAPI) database that receives a query asking for a property of a material and then retrieves the relevant information from the dataset. If the material is not available on MAPI, the agent can search for similar materials and use in-context learning (ICL) to provide a prediction of the requested property. Additionally, MAPI\_LLM also has a reaction module for synthesis proposal. Second, \citet{Rankovic2023-bd} used LLMs to make BO algorithms more accessible to a broader group of scientists; BOLLaMa implements a natural language interface to easily interact with BO software developed by their group\cite{Rankovic2023-qo}. Third, and similar to \citet{Ramos2023-cs} and \citet{Rankovic2023-ge} who employed LLMs in BO, \citet{Weiser2023-ac} focused on genetic algorithms (GA), a different optimization algorithm. In GA, pieces of information are stochastically combined and evaluated to guide the algorithm during the optimization. For chemistry, these pieces are often molecular fragments that are combined to compose a final whole molecular structure. Thus, \citet{Weiser2023-ac} used LLMs to implement common GA operators under the hypothesis that LLMs can generate new combined molecules better than random cross-over due to their sensory memory. Fourth, InsightGraph\cite{Circi2023-ja} can draw general relationships between materials and their properties from JSON files. \citet{Circi2023-ja} showed that LLMs can understand the structured data from a JSON format and reorganize the information in a knowledge graph. Further refinement of this tool could automate the process of describing relationships between materials across various scientific reports, a task that remains labor-intensive today. Fifth, \citet{Kruschwitz2023-da} used ICL and LLMs to accurately predict the compressive strength of concrete formulations; Text2Concrete achieved predictive accuracy comparable with a Gaussian process regression (GPR) model, with the advantage that design principles can be easily added as context. This model was successfully applied in a BO algorithm following \citet{Ramos2023-cs} approach.\cite{Volker2024-nv}
For education purposes, multiple authors have raised the discussion about how LLMs can be used to support educators' and instructors' daily work.\cite{Zaabi2023-mx, Kasneci2023-oh, Hellas2023-ks, Dan2023-gs, Tian2024-en} Finally, in this direction, \citet{Mourino2023-fj} developed i-Digest, an agent whose perception module can understand audio tracks and video recordings. These audio recordings are transcribed to text using the Whisper\cite{Radford2022-wq} model, and therefore, i-Digest is a digital tutor that generates questions to help students test their knowledge about the course material. These are just a few examples to showcase the capabilities of AI systems to innovate and generate solutions rapidly.

More recently, \citet{Ma2024-no} showed that agents can be trained to use tools. SciAgent\cite{Ma2024-no} was developed under the premise that finetuning LLMs for domain-specific applications is often impractical. Nevertheless, the agent can be fine-tuned with a set of tools that will enable them to perform well in a domain-specific task. These tools, typically Python functions, enable SciAgent to plan, retrieve, and use these tools to facilitate reasoning and answer domain-related questions effectively. The benchmark developed for SciAgent, known as \texttt{SciToolBench}, includes five distinct domains, each equipped with a set of questions and corresponding tools. The development of its retrieval and planning modules involved finetuning different LLMs on the MathFunc benchmark, resulting in a notable performance improvement of approximately $\sim$~20\% across all domains in \texttt{SciToolBench} compared to other LLMs.

\subsection{Agents for literature review}

Another fantastic opportunity for automation in the sciences is associated with high-quality literature review, a pivotal aspect of scientific research that requires reading and selecting relevant information from large numbers of papers, and thereby distilling the current state of knowledge relevant to a particular research direction. This extremely time-consuming task is being revolutionized by advanced AI tools designed to automate and enhance such analysis and summarization.

PaperQA introduces a robust model that significantly reduces misinformation while improving the efficiency of information retrieval. This agent retrieves papers from online scientific databases, reasons about their content, and performs question-answering (QA) tasks. Its mechanism involves three primary components—"\texttt{search}", "\texttt{gather\_evidence}", and "\texttt{answer\_question}" and the authors adapted the Retrieval-Augmented Generation (RAG)\cite{Lewis2020-bh} algorithm to include inner loops on each step. For instance, PaperQA can perform multiple rounds of \texttt{search} and \texttt{gather\_evidence} if, with reflection, not have enough evidence has been acquired to successfully \texttt{answer\_question}.
Further validating its capabilities, a new benchmark called LitQA demonstrates that PaperQA not only meets but exceeds human performance in solving complex, real-world scientific questions. By applying the RAG technique to full-text scientific papers, PaperQA sets a new standard in QA capabilities, achieving human-like performance in curated datasets without hallucination or selecting irrelevant citations.\cite{Lala2023-ru} To further investigate PaperQA performance, the authors developed a new benchmark called LitQA, which designs tasks that mimic the complexity of real scientific inquiry. The benchmark comprises 50 multiple-choice questions sourced from biomedical papers published post-September 2021, ensuring they were not part of the LLM training data. In this setting, PaperQA demonstrated a precision rate of 87.9\% and surpassed typical human accuracy, scoring 69.5\% compared to 66.8\%.\cite{Lala2023-ru}

Building on top of PaperQA, WikiCrow exemplifies the practical application of AI in generating concise and relevant Wikipedia-style summaries. The authors show that while 16\% of a human-created Wikipedia article comprises irrelevant statements, WikiCrow displays irrelevant information only 3\% of the time. Their system also added 5\% more correct citations when compared with original articles. Moreover, thanks to its foundation in the PaperQA framework\cite{Lala2023-ru}, WikiCrow achieves remarkable cost-efficiency. The authors estimate that WikiCrow can accomplish in a few days what would take humans approximately 60,000 hours, or about 6.8 years, thereby underscoring its ability to rapidly produce extensive scientific content. This efficiency exemplifies the reliability and transformative potential of AI in content creation \cite{wikicrow2024}.

Following a different approach, the STORM model also addressed the problem of writing Wikipedia-like summaries, where the STORM acronym represents the Synthesis of Topic Outlines through Retrieval and Multi-perspective questions.\cite{Shao2024-qk} This approach implements a two-step procedure. First, STORM retrieves multiple articles on a topic and uses an LLM to integrate various perspectives into a cohesive outline. Second, this outline is used to write each section of the Wikipedia-like summary individually.
To create the outline, multiple articles discussing the topic of interest are retrieved by an "expert" LLM, which processes each one to create $N$ perspectives. Each perspective is then fed to a "writer" LLM, and a conversation is initiated between writer and expert. Finally, the $N$ conversations are used to design the final outline.
The outline and the set of references, accessed by RAG, are given to the writer LLM. The writer LLM is prompted to use these inputs to generate each section of the article sequentially. Following this, all sections are merged and refined to eliminate redundancies and enhance coherence. Upon human evaluation, STORM is reported to be $\sim$~25\% more organized and present $\sim$~10\% better coverage when compared to a pure RAG approach. However, it was also less informative than human-written Wikipedia pages, and STORM presented a transfer of internet-borne biases, producing emotional articles, which is a major concern.

Ultimately, the idea of an ``AI scientist'' who can generate new, relevant research questions (RQ) has been pursued. Aligned with this vision, \citet{Liu2023-ye} developed CoQuest, partially automating the brainstorming for new RQs process. This system uses a human-computing interface (HCI) to allow the agent to create new RQs that can be further enhanced by human feedback. They developed two strategies for RQ generation: breadth-first, where the agent generates multiple RQs simultaneously following the original user's prompt, and depth-first, where multiple RQs are created sequentially, building on the top of the previously generated RQ. For each RQ generation, the agent implements a ReAct\cite{Yao2022-db} framework with tools for literature discovery, hypothesis proposition, refinement, and evaluation. Upon evaluation of 20 HCI doctoral researchers by a post-interaction survey, the breadth-first approach was preferred by 60\% of the evaluators. Interestingly, despite the evaluators' report that the breadth-first approach gave them more control and resulted in more trustworthy RQs, the depth-first had better scores for novelty and surprise. This difference might be caused by the fact that the depth-first uses its own RQ to iterate. This process can introduce new keywords not considered by the users.

\subsection{Agents for chemical innovation}

Transitioning from literature synthesis to practical chemistry applications, we next explore how LLM-based agents have proven their capabilities to revolutionize routine chemical tasks towards an acceleration of molecular discovery and scientific research. Agents are flexible entities capable of developing prompt-specific workflows and executing a plan toward accomplishing a specific task. ChemCrow\cite{Bran2023-jk} introduced a significant shift in how LLMs would be applied in chemistry, given that LLMs alone do not access information outside of their training data nor can they directly perform chemistry-related tasks. 

By augmenting LLMs with common chemical tools, computational or robotic, ChemCrow automates a broad spectrum of routine chemical tasks, demonstrating a significant leap in LLM applicability. Under human evaluation, ChemCrow consistently outperformed GPT-4, achieving an accuracy score of 9.24/10 compared to 4.79/10.\cite{Bran2023-jk}
The developers of ChemCrow have also considered the ethical implications and potential risks associated with its capabilities. ChemCrow's high potential could be misused and exploited for malicious objectives, and therefore the authors have implemented safety checks and guidelines to prevent such misuse, or "dual usage". Additionally, they acknowledge that ChemCrow, relying on an LLM, may not always provide completely accurate answers due to gaps in its chemical knowledge. As such, they recommend careful and responsible use of the tool, along with thorough scrutiny of its outputs. In summary, while ChemCrow presents a powerful new chemical assistant\cite{Bran2023-jk}, oversight of its use is required, and this agent's access to tools has been deliberately limited to enhance security and avoid misuse.

Similarly to ChemCrow\cite{Bran2023-jk}, Chemist-X\cite{Chen2023-cg} uses RAG to get up-to-date literature information and use it to reliably solve user's questions. Nevertheless, Chemist-X focuses on designing chemical reactions to achieve a given molecule. It works in three phases: (1) First, the agent searches molecule databases for similar molecules, then (2) there is a look-up for online literature searching for chemical reactions capable of converting the list of similar molecules in the target. Lastly, (3) machine learning models are used to propose the reaction conditions. To validate their agent, the authors used Chemist-X to design an HTS experiment aiming to produce 6-(1-methyl-1H-indazol-4-yl), resulting in a maximum yield of 98.6\%.

On the other hand, the Coscientist\cite{Boiko2023-ot} system exemplifies the integration of semi-autonomous robots in planning, conceiving, and performing chemical reactions with minimal human intervention. At its core, the system features a main module named `PLANNER', which is supported by four submodules. These submodules, or tools, are responsible for performing actions such as searching the web for organic synthesis, executing Python code, searching the hardware documentation, and performing a reaction in an automated lab.\cite{Boiko2023-ot} Utilizing this framework, the Coscientist successfully conducted two types of chemical coupling reactions, Suzuki-Miyaura and Sonogashira, in a semi-automated fashion, with manual handling of initial reagents and solvents. Additionally, Coscientist was also used to optimize reaction conditions.
In contrast to \citet{Ramos2023-cs}, who used LLMs within a Bayesian Optimization (BO) algorithm as a surrogate model, \citet{Boiko2023-ot} approached the optimization task as a strategic "game" aimed at maximizing reaction yield by selecting optimal reaction conditions. This demonstrates the ability of GPT-4 to effectively reason about chemical reactions.
The authors have indicated that the code for their agent will be released following changes in U.S. regulations on AI and its scientific applications. At the time of writing, the code remains unreleased, but a simple example that calculates the square roots of random numbers has been provided to illustrate their approach.\cite{Boiko2023-ot}.
These examples underscore the transformative role of LLMs in enhancing and automating chemical processes, which will likely accelerate chemical discovery.

Automated workflows in protein research have also been explored. ProtAgent\cite{Ghafarollahi2024-kj} is a multi-agent system designed to automate and optimize protein design with minimal human intervention. This system comprises three primary agents: \texttt{Planner}, \texttt{Assistant}, and \texttt{Critic}. The \texttt{Planner} is tasked with devising a strategy to address the given problem, the \texttt{Assistant} executes the plan using specialized tools and API calls, and the \texttt{Critic} supervises the entire process, providing feedback and analyzing outcomes. These agents collaborate through a dynamic group chat managed by a fourth agent, the \texttt{Chat Manager}. Tasks executed by this team include protein retrieval and analysis, \textit{de novo} protein design, and conditioned protein design using Chroma\cite{Ingraham2023-hf} and OmegaFold\cite{Wu2024-mc}.

Similarly to ProtAgent, \citet{Liu2024-xm} created a team of AI-made scientists (TAIS) to scientific discovery without human intervention. However, their agents have roles analog to human roles in scientific discovery, for instance, project manager, data engineer, code reviewer, statistician, and domain expert. While in ProtAgent\cite{Ghafarollahi2024-kj} agents interact through the \texttt{Chat Manager} only, TAIS\cite{Liu2024-xm} enables AI scientists to interact between themselves directly using pre-defined collaboration pipelines. To evaluate TAIS, the authors curated the Genetic Question Exploration (GenQEX) benchmark, which consists of 457 selected genetic data questions. As a case study, the authors show TAIS's answer to the prompt \texttt{"What genes are associated with Pancreatic Cancer when considering conditions related to Vitamin D Levels?"}. The system identified 20+ genes with a prediction accuracy of 80\%. 

The agents in chemistry, as exemplified by ChemCrow\cite{Bran2023-jk} and Coscientist\cite{Boiko2023-ot}, highlight a significant shift towards automation and enhanced efficiency in molecular discovery and scientific research. These systems demonstrate the potential of integrating LLMs with chemical tools and automation frameworks, achieving impressive accuracy and effectiveness in tasks ranging from routine chemical operations to complex reaction optimizations. Similarly, ProtAgent\cite{Ghafarollahi2024-kj} and TAIS\cite{Liu2024-xm} systems showcase the versatility of multi-agent frameworks in automating protein design and genetic research, pushing the boundaries of what AI-driven scientific discovery can achieve. These studies collectively showcase the incredible potential of agents in chemical and biological research, promising automation of routine tasks, easing the application of advanced techniques and analyses, and accelerating discoveries. However, they also underscore the necessity for meticulous oversight and responsible development to harness their full potential while mitigating risks.\cite{Tang2024-nx}


\subsection{Agents for experiments planning}

Building on the capabilities of ChemCrow and Coscientist in automating chemistry-related tasks, recent advances have focused on bridging the gap between virtual agents and physical laboratory environments.
For example, Context-Aware Language Models for Science (CALMS)\cite{Prince2023-ar}, BioPlanner\cite{ODonoghue2023-tx}, and CRISPR-GPT\cite{Huang2024-pg} focus on giving support to researchers with wet-lab experimental design and data analysis.

CALMS\cite{Prince2023-ar} focuses on improving laboratory efficiency through the operation of instruments and management of complex experiments, employing conversational LLMs to interact with scientists during experiments. In addition, this agent can perform actions using lab equipment after lab equipment APIs have been provided to the agent as tools. 
% The developers of CALMS, \citet{Prince2023-ar}, emphasize the increasing complexity and intricacy of laboratory equipment, necessitated by advanced experimental demands. 
CALMS was designed to enhance instrument usability and speed up scientific discovery, providing on-the-spot assistance for complex experimental setups, such as tomography scans, and enabling fully automated experiments. For instance, its capability was showcased through the operation of a real-world diffractometer. Although CALMS excelled in several tasks, a comparison between GPT-3.5 and Vicuna 1.5 revealed Vicuna's limitations in handling tools.

In contrast, BioPlanner\cite{ODonoghue2023-tx} significantly improves the efficiency of scientific experimentation by creating pseudocode representations of experimental procedures, showcasing AI's capacity to streamline scientific workflows. Therefore, Rather than interacting directly with lab equipment through APIs, BioPlanner creates innovative experimental protocols that can be expanded upon within a laboratory setting.
The initial step in BioPlanner's process involves assessing the capability of LLMs to produce structured pseudocode based on detailed natural language descriptions of experimental procedures.
% Using either GPT-3 or GPT-4, the system breaks down the overall task into smaller, manageable subtasks. For each subtask, the models generate a specific function. These functions are then integrated to complete the overarching experimental procedure. 
In testing, BioPlanner successfully generated correct pseudocode for 59 out of 100 procedures using GPT-4, although the most common errors involved omitted units.
Afterward, the authors used BioPlanned to generate a procedure for culturing an E.coli bacteria colony and storing it with cryopreservation, which ran successfully.

% Their manually verified dataset, rigorously checked and confirmed, was compiled and named BioProt. BioProt serves to further verify the LLMs' ability to devise functional experimental protocols. Leveraging this dataset, an LLM-based agent equipped with BioProt pseudofunctions was created to test these protocols in practical scenarios. BioPlanner successfully generated an experimental procedure when prompted, it would be "culturing a single colony of E.coli bacteria overnight and making a glycerol stock with the suspension (a form of cryopreservation for long-term storage)."

Focusing on gene editing experiments, CRISPR-GPT\cite{Huang2024-pg} is an agent developed to design experiments iteratively with constant human feedback.
% Gene editing allows precise alteration of DNA in living organisms, with extensive applications in biology and medicine. One well-known system is CRISPR-Cas9, but designing CRISPR experiments requires numerous considerations typically handled by specialists. 
CRISPR-GPT\cite{Huang2024-pg} aims to bridge the gap for non-experts by simplifying this process into manageable steps solvable by an LLM with access to useful tools. This agent operates in three modes based on user prompts: ``Meta mode'' provides predefined pipelines for common gene-editing scenarios; ``Auto mode'' uses the LLM to plan a sequence of tasks; and "Q\&A mode" answers general questions about the experimental design. The authors demonstrate that based on human evaluations, CRISPR-GPT outperforms GPT-3.5 and GPT-4 in accuracy, reasoning, completeness, and conciseness. Additionally, they applied CRISPR-GPT to design real-world experiments for knocking out TGFBR1, SNAI1, BAX, and BCL2L1 in the human A375 cell line, achieving an editing efficiency of approximately 70\% for each gene.

Following the ideas of developing agents for automating experimental protocol generation, \citet{Ruan2024-lw} created a multi-agents system composed of 6 agents: \texttt{Literature Scouter}, \texttt{Experiment Designer}, \texttt{Hardware Executor}, \texttt{Spectrum Analyzer}, \texttt{Separation Instructor}, and \texttt{Result Interpreter}. The Large Language Models-based Reaction Development Framework (LLM-RDF)\cite{Ruan2024-lw} automates every step of the synthesis workflow. While other studies focus on the literature review\cite{Zheng2023-ka, Zhang2024-ab, Zheng2024-oz}, HTS\cite{Chen2023-cg}, and reaction optimization\cite{Zheng2023-gb, Boiko2023-ot}, LLM-RDF can support researchers from literature search until the product purification. Using this system, the authors showed they could design a copper/TEMPO catalyzed alcohol oxidation reaction, optimize reaction conditions, engineer a scale-up, and purify the products, obtaining a yield of 86\% and a purity >98\% while producing 1 gram of product. 

Interestingly, despite acting on different fields and presenting different goals (while CALMS\cite{Prince2023-ar} and LLM-RDF\cite{Ruan2024-lw} can autonomously use laboratory equipment, BioPlanner\cite{ODonoghue2023-tx} and CRISPR-GPT\cite{Huang2024-pg} propose a protocol that needs to be carried out by a human), all studies implemented a ``human-in-the-loop'' approach. Maintaining the researcher a vital piece of the development is a way to enhance reliability and mitigate agent limitations, such as errors and hallucinations. This approach also addresses risk and dual usage problems once a human can decide whether the agent's suggestions are safe. \cite{Wang2023-kc, Nascimento2023-vo}

\subsection{Agents for automating cheminformatics tasks}

Cheminformatics consists of applying information technology techniques to convert physicochemical information into knowledge. The process of solving cheminformatics problems commonly involves retrieving, processing, and analyzing chemical data.\cite{Niazi2023-is}
Getting inspiration from ChemCrow\cite{bran_chemcrow_2023} ideas, Chemistry Agent Connecting Tool Usage to Science (CACTUS)\cite{McNaughton2024-qj} focused on assisting scientists by automating cheminformatics tasks. CACTUS automates the applications of multiple cheminformatics tools, such as property prediction and calculation, while maintaining the human-in-the-loop for molecular discovery. The authors investigated the performance of a diverse set of open-source LLMs, where Gemma-7B and Mistral-7B demonstrated superior performance against LLaMA-7B and Falcon-7B. In addition, the authors reported that adding domain-specific information in the prompt to align the agent to chemistry problems considerably increases model's performance. For instance, predicting drug-likeness with a Gemma-7B agent improves the accuracy of  $\sim$ 60\% when aligning the agent. Prompt alignment improved the prediction of all properties they studied.

Further illustrating the versatility of AI in scientific research and domain-specific tools usage is ChatMOF,\cite{Kang2023-zs} which focuses on the prediction and generation of Metal-Organic Frameworks (MOFs). ChatMOF integrates MOF databases with its MOFTransformer\cite{Kang2023-xd} predictor module, thereby showcasing the innovative use of genetic algorithms in guiding generative tasks from associated predictions. The authors showed that ChatMOF achieved an accuracy of $\sim$~90\% in search and prediction tasks while generative tasks have an accuracy of $\sim$~70\%. The genetic algorithm used by ChatMOF allows for the generation of a diverse array of MOF structures, which can be further refined based on specific properties requested by users. For instance, when prompted to, ``generate structures with the largest surface area'', the system initially generated a broad distribution of structures with surface area centered in 3784 m$^2$/g, and the GA evolves it to a narrower distribution with a peak at 5554 m$^2$/g after only three generations. It is important to note that even though ChatMOF has access to a dataset of experimental values for MOFs, language model predictions guide their GA, and no further validation has been made.
Lastly, \citet{Ansari2023-qi} developed Eunomia, another domain-specific autonomous AI agent that leverages existing knowledge to answer questions about materials. Eunomia\cite{Ansari2023-qi} can use chemistry tools to 
access a variety of datasets, scientific papers and unstructured texts to extract and reason about material science information. The authors implemented a CoVe\cite{Dhuliawala2023-wp} (Consistency Verification) scheme to evaluate the model's answer and minimize hallucination. The authors showed that including CoVe increased the model's precision by $\sim$~20\% when compared to previous methods such as an agent using ReAct only.\cite{Yao2022-db}

Promoting molecular discovery is a topic with great attention in the literature devoted to it and, as described extensively above, LLMs have leveraged a large amount of unstructured data to accelerate that discovery. \citet{Janakarajan2023-fk} discuss the advantages of using LLMs in fields such as \textit{de novo} drug design, reaction chemistry, and property prediction, but they augment the LLM in \texttt{IBM ChemChat}, a chatbot with the capability of using common APIs and python packages commonly used daily by a cheminformatics researcher to access molecular information. \texttt{ChemChat} has access to tools such as Generative Toolkit for Scientific Discovery (GT4SD)\cite{Manica2023-hv}, a package with dozens of trained models generative models for science, rxn4chemistry\cite{rxn4chemistry}, a package for computing chemistry reactions tasks, HuggingMolecules\cite{Gainski2022-an}, a package developed to aggregate molecular property prediction LMs, and RDKit\cite{Landrum2013-nt}, a package to manipulating molecules. Since \texttt{ChemChat} implements an agent in a chat-like environment, users can interactively refine design ideas. Despite being developed to target \textit{de novo} drug design, \texttt{ChemChat} nonetheless is a multi-purpose platform that can be more broadly used for molecular discovery.

In addition to the capabilities described above, LLM-based agents can empower users to tackle tasks that typically require extensive technical knowledge. In previous work, \citet{Wellawatte2023-rw} and \citet{Gandhi2022-mx} showed that including natural language explanations (NLE) in explainable AI (XAI) analysis can improve user understanding. More recently, \citet{Wellawatte2023-rw} developed XpertAI\cite{Wellawatte2023-rw} to seamlessly integrate XAI techniques with LLMs to interpret and explain raw chemical data autonomously. Applying XAI techniques is usually restricted to technical experts but by integrating such techniques with an LLM-based agent to automate the workflow, the authors made XAI accessible to a wider audience.

Their system receives raw data with labels for physicochemical properties. The raw data is used to compute human-interpretable descriptors and then calculate SHAP values or Z-scores for Local Interpretable Model-agnostic Explanations (LIME). By calculating SHAP values (or SHapley Addictive exPlanations) a value can be assigned to each feature, indicating its contribution to a model’s output. LIME interprets a model by making a local approximation, around a particular prediction, to indicate what factors have contributed to that prediction in the model. It may use, for example, a surrogate local linear regression fit to recognized features.\cite{Gandhi2022-mx}
In addition to XAI tools, XpertAI can search and leverage scientific literature to provide accessible NLEs.
While ChatGPT provides scientific justifications with similar accuracy, its explanation is often too broad. On the other hand, XpertAI provides data-specific explanations and visual XAI plots to support its explanations.\cite{Wellawatte2023-rw}

These developments signify a growing trend in the integration of tools and LLMs in autonomous AI within scientific research. By automating routine tasks, enhancing information retrieval and analysis, and facilitating experimentation, AI is expanding the capabilities of researchers and accelerating the pace of scientific discovery. This review underscores the transformative impact of AI across various scientific domains, heralding a new era of innovation and efficiency in chemical research.

\section{Challenges and opportunities}

LLMs hold great potential in chemistry due to their ability to both predict properties and orchestrate existing computational and experimental tools. These capabilities enhance the accuracy and efficiency of chemical research and open up new avenues for discovery and innovation. By encapsulating AI models, data analysis software, and laboratory equipment within agent-based frameworks, researchers can harness these sophisticated tools through a unified interface. This approach not only simplifies the interaction with complex systems but also democratizes the immense capabilities of modern computational tools, thereby maximizing their utility in advancing chemical research and development.

\paragraph{Data Quality and Availability} 
Quality and availability of data are critical factors that influence the efficacy of LLMs. Indeed, scaling both the model size and the amount of training data used has proven to improve capabilities.\cite{OpenAI2023-md} However, current AI models are not trained on large amounts of chemical data, which limits their capabilities to reason about advanced chemical concepts.\cite{Mirza2024-qw}

There are two types of datasets commonly used to train LLMs: unlabeled and labeled datasets.
Unlabeled datasets, or pretraining data, are used during the semi-supervised training, which focuses on creating a ``prior belief'' about a molecule. Currently, we have huge datasets composed of hypothetical and/or theoretical data. When a model is trained on data that is not grounded in real chemical information, this might cause the model to learn a wrong prior belief.\cite{Gao2020-ey}
% For instance, the Chembl\cite{Gaulton2012-og} dataset is a manually curated dataset of bio-active drug-like molecules with calculated properties. On the other hand, ZINC\cite{irwin2012zinc} dataset contains commercially available molecules and a subset of hypothetical molecules that can, theoretically, be synthesized. 

Labeled datasets, often used in benchmarks, also suffer from their inclusion of hypothetical and calculated data. Benchmarks are necessary for quantifying improvements in AI modeling and prediction within a competitive field. However, dominant benchmarks like MoleculeNet,\cite{wu_moleculenet_2018} have significant limitations that may restrict the generalizability and applicability of evolving models. In his blog, \citet{pat_walters_blog3} brings to light numerous errors and inconsistencies within the MoleculeNet data, which substantially impact model performance and reliability.\cite{Gloriam2019-yf, irwin_chemformer_2022, liu_multi-modal_2023, Livne2023-bu}. Walters also argues that the properties present in these benchmarks do not directly correlate with real chemistry improvement. As such, new benchmarks need to translate to practical chemistry problems directly. For instance, increasing accuracy in predicting LogP is not necessarily mapped to drugs with greater bioavailability. Some promising work has come from the Therapeutic Common Data (TDC)\cite{Huang2021-ug, TDC-ss} includes data from actual therapeutic essays, providing a more practical foundation for model training. 

The community continues to work to organize and curate datasets to make data ready for LLMs training and evaluation. Scientific benchmarks\cite{Peng2019-yb, Lala2023-ru, Liu2024-hv}, repositories with curated datasets\cite{_jablonka_awesome-chemistry-datasets}, and packages for model evaluation\cite{Mirza2024-qw} have been developed.
However, the challenges concerning grounded truth and consistent datasets remain.
With advancements in scientific document processing,\cite{Swain2016-se} there is now the opportunity to obtain new datasets from peer-reviewed scientific papers.
Due to the multi-modal capabilities of such AI models, these new benchmarks can comprise multiple data types, potentially enhancing the applicability and transferability of these models. The continual curation of new, relevant datasets that represent the complexities of real-world chemical problems will further enhance the robustness and relevance of LLMs in chemistry.

% One continuing challenge in deploying LLMs in chemistry is the quality and accessibility of data. Training on calculated data introduces some abstraction from real-world properties.\cite{irwin_chemformer_2022} Therefore, incorporating more experimentally derived data into Chemistry LLM research is critical for developing more robust and relevant models. Continual curation of new, relevant datasets that represent the complexities of real-world chemical problems will enhance the applicability and transferability of these models.

\paragraph{Model Interpretability} Model interpretability is a significant challenge for LLMs due to their ``black-box'' nature, which obscures the understanding of how predictions are made.
However, innovative approaches are being developed to enhance LLMs' interpretability. For instance,\citet{Schilter2023-ux} used information from the different multi-attention heads to assign H-NMR peaks to specific hydrogens in a molecule, so as to indicate how spectra were comprehended or structures deduced. Additionally, since the LLMs use language, which is intrinsically interpretable, LLMs may be incrementally modified to explain their reasoning processes directly, exemplified with tools like eXpertAI\cite{Wellawatte2023-rw} and or simply adjusting prompting\cite{Wei2022-rm, Chen2023-df}. These methods address the critical need for transparency in the mechanism of understanding for a good prediction beyond the good prediction itself.

\paragraph{Integration with Domain Knowledge and Cross-disciplinary Applications} While LLMs excel at pattern recognition, integrating explicit chemical rules and domain knowledge into these systems remains challenging. This integration is essential to make predictions that are not only statistically valid but also chemically reasonable. It was shown by \citet{Beltagy2019-ri} and \citet{Gu2021-yn} that better performance on common NLP tasks can be achieved by developing a vocabulary and pretraining on a domain-specific training corpus. While, pretrainng with domain-specific datasets that include chemical properties, reaction mechanisms, and experimental results may better capture the nuances of chemistry, the challenge to use AI to promote multi-disciplinary research remains. The Galactica LLM \cite{Taylor2022-pu} also used special tokens for delineating chemical information, to relatively good success on chemistry tasks. \citet{Aryal2024-na} also progress by creating an ensemble of specialist agents with different domains of knowledge, allowing them to interact to better answer the user query. Specifically, \citet{Aryal2024-na} used agents with chemistry, physics, electrochemistry, and materials knowledge. 
%The whole concept of autonomous agents, based on the integration and collaboration of specialized tools further highlights the power of such agents to provide depth of knowledge and multi-domain versatility, and is a significant opportunity indicated for further research in the field. 
%However, these concepts could be extended even for a multi-domain approach.
% \paragraph{Scalability and Computational Resources} The training and deployment of LLMs require substantial computational resources, which can be a limiting factor. 

\paragraph{Tool development}

The effectiveness of a combined LLM/Autonomous Agent approach hinges significantly on the availability and quality of the tools, as well as on the complexity and diversity of the chemical tasks at hand.
Some emphasis should be placed on refining standalone tools, with the confidence that overarching frameworks, like a GPT-4-type wrapper, or "assistant", will eventually integrate these tools seamlessly. Developers should stay informed about existing tools and design their tools to interface effectively with such a wrapper. This ensures that each tool is ready to contribute its unique capabilities to a cohesive agent system.

\paragraph{Reinforcement learning} Reinforcement learning has been successfully used in LLMs\cite{Bohm2019-ue, Pan2023-lb, OpenAI2022-RLHF}, with a few applications also proposed for use in agents\cite{Hu2023-sw, Xu2023-et}. However, no study involving using RL to optimize agents to perform better in scientific tasks dynamically has yet been developed. Implementing some of these RL concepts in the context of agents might allow the systems to dynamically adapt to new problems and significantly reduce hallucination even in domains where the core LLM was not sufficiently pre-trained.


\paragraph{Agent evaluation} Comparing different agent systems is challenging due to the lack of robust benchmarks and evaluation schemes. Consequently, it is difficult to define what constitutes a ``superhuman'' digital chemist and reach a consensus on the criteria for success. This issue is similar to the ongoing discussions about defining artificial general intelligence (AGI) and the expected capabilities of cognitive architectures.\cite{Langley2009-eh, Goertzel2014-nm}
Once a reliable metric for evaluating such AI systems is established, it is crucial for the AI scientific community to set clear guidelines for conducting research. Currently, assessing success is challenging because the goals are not well defined. Building on this, we propose using Bloom’s taxonomy as a reference point for developing a metric to evaluate more complex reasoning and tool use in autonomous agents. This educational framework categorizes cognitive skills in a hierarchical manner, from basic recall to creative construction, providing a structured approach to assess higher-order thinking and reasoning capabilities in these systems. This adaptation could significantly enhance the evaluation of LLMs and autonomous agents, especially when tackling complex chemical challenges.

\paragraph{Ethical and Safety Concerns} As with all AI technologies, there are ethical considerations in deploying LLMs, including bias in model predictions and the potential misuse of AI-generated chemical knowledge. \citet{Ruan2023-oq} and \citet{Tang2024-nx} pointed out the necessity of different levels of regulation in agent development, noting that current alignment methods may be insufficient for ensuring safety,
%. They showed that using alignment methods for promoting LLM safety might not be enough to promote agent safety.
and using human evaluation to address the risks of such systems is not scalable. Therefore, the lack of specialized models for risk control and effective safety evaluations poses perhaps the greatest challenges when assuring the safety of LLMs with the ability to use tools. This underscores the urgency, and the opportunity, in automating red-teaming of agents to enhance safety protocols in AI technologies.

\paragraph{Human-AI Collaboration in Chemical Research}

LLMs are poised to transform fields such as drug discovery, materials science, and environmental chemistry due to their ability to predict chemical properties and reactions with remarkable accuracy. Models based on architectures like BERT have demonstrated their capability to achieve state-of-the-art performance in various property prediction tasks.\cite{li_mol-bert_2021,wang_smiles-bert_2019} Furthermore, studies by \citet{Jablonka2023-bm} and \citet{born_regression_2023} have showcased the predictive power of LLMs by reformulating traditional regression and classification tasks as generative tasks, opening up new avenues for chemical modeling. However, as emphasized by \citet{Weng2023-ic}, maintaining the reliability of LLM outputs is essential, as inaccuracies in formatting, logical reasoning, or content can significantly impede their practical utility.
Hallucination is also an intrinsic issue with LLMs.\cite{Ji2023-cg} Though agents can deal with hallucinations to some extent by implementing sanity-checking tools, it does not make the response hallucination-proof. A possible approach to address this issue is to use a human-in-the-loop approach, where steps of human-agent interaction are added to the workflow to check if the agent is in the correct pathway to solve the request.\cite{Cai2023-pw, Xiao2023-qg, Drori2024-pk}

The potential of LLMs to design novel molecules and materials was highlighted by the AI-powered robotic lab assistant, A-Lab, which synthesized 41 new materials within just 17 days.\cite{szymanski_autonomous_2023} Nonetheless, this achievement has sparked debates about the experimental methods and the actual integration of atoms into new crystalline materials, raising questions about the authenticity of the synthesized structures.\cite{peplow_robot_2023} These controversies underline the necessity for rigorous standards and the critical role of human expertise in validating AI-generated results. Again, the integration of advanced AI tools with the oversight of seasoned chemists is crucial, suggesting that a hybrid approach could significantly enhance both the innovation and integrity of materials science research.

In parallel, we have seen how LLM-based agents are increasingly capable of automating routine tasks in chemical research, which traditionally consume significant time and resources. These models excel in real-time data processing, managing vast datasets, and even conducting comprehensive literature reviews with minimal human intervention. Advances in AI technology now allow agents not only to perform predefined tasks but also to adapt and develop new tools for automating additional processes. For instance, tasks such as data analysis, literature review, and elements of experimental design are now being automated.\cite{Wellawatte2023-rw, Hong2024-lg, Qi2024-qe, Lala2023-ru, ODonoghue2023-tx, Prince2023-ar, Bran2023-jk, Boiko2023-ot} This automation liberates chemists to focus on more innovative and intellectually engaging aspects of their work, and the opportunity is to expand productivity and creativity in their science.

\section{Conclusions}

Since this review is targeted in part to an audience of chemists, who may not have yet embraced AI technology, we consider it valuable to point out our perspective that AI in chemistry is definitely here to stay. The dot-com boom led to a substantial change in the workforce, followed by a bust but ultimately leading to an entirely new industry of online commerce and connectivity. AI is no different a technology disruptor in that regard, and it has already been adopted behind the scenes by many corporations. We therefore predict that it will only grow in its use as a necessary tool that will inevitably lead to more jobs and greater progress. We therefore hope to facilitate the change by connecting the technology to the chemical problems that our readership is already addressing through more traditional methods.

Large Language Models (LLMs) have demonstrated remarkable potential in reshaping chemical research and development workflows.
These models have facilitated significant advancements in molecular simulation, reaction prediction, and materials discovery.
In this review, we discussed the evolution of LLMs in chemistry and biochemistry.
Successful cases where LLMs have proven their potential in promoting scientific discovery were shown with caveats of such models.

Adopting LLM-based autonomous agents in chemistry has enhanced the accuracy and efficiency of traditional research methodologies and introduced innovative approaches to solving complex chemical problems. 
Looking forward, the continued integration of LLMs promises to accelerate the field's evolution further, driving forward the frontiers of scientific discovery and technological innovation in chemistry. 
We have shown how agents have been used in chemistry and proposed a framework for thinking about agents as a central LLM followed by interchangeable components. 

However, despite the community's already astonishing advances in this field, many challenges still require solutions. 
We pointed out the main challenges and opportunities we identify that need to be addressed to promote further development of agents in chemistry.
Addressing the challenges related to model transparency, data biases, and computational demands will be crucial for maximizing their utility and ensuring their responsible use in future scientific endeavors.

While there are significant challenges to be addressed, the opportunities presented by LLMs in chemistry are vast and have the potential to alter how chemical research and development are conducted fundamentally. Effectively addressing these challenges will be crucial for realizing the full potential of LLMs in this exciting field.
To keep pace with the ever-growing, we will maintain a repository with an organized structure listing new studies regarding LLMs and LLM-based agents focused on scientific purposes.
The repository can be found in \url{https://github.com/ur-whitelab/LLMs-in-science}
